Reinforcement Learning in Non-Stationary Discrete-Time Linear-Quadratic Mean-Field Games

In this paper, we study large population multi-agent reinforcement learning (RL) in the context of discrete-time linear-quadratic mean-field games (LQ-MFGs). Our setting differs from most existing work on RL for MFGs, in that we consider a non-stationary MFG over an infinite horizon. We propose an actor-critic algorithm to iteratively compute the mean-field equilibrium (MFE) of the LQ-MFG. There are two primary challenges: i) the non-stationarity of the MFG induces a linear-quadratic tracking problem, which requires solving a backwards-in-time (non-causal) equation that cannot be solved by standard (causal) RL algorithms; ii) Many RL algorithms assume that the states are sampled from the stationary distribution of a Markov chain (MC), that is, the chain is already mixed, an assumption that is not satisfied for real data sources. We first identify that the mean-field trajectory follows linear dynamics, allowing the problem to be reformulated as a linear quadratic Gaussian problem. Under this reformulation, we propose an actor-critic algorithm that allows samples to be drawn from an unmixed MC. Finite-sample convergence guarantees for the algorithm are then provided. To characterize the performance of our algorithm in multi-agent RL, we have developed an error bound with respect to the Nash equilibrium of the finite-population game.

==> Section3_add.tex <==
XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX

{\color{blue}We now present the actor-critic (which forms the inner loop in Algorithm \ref{alg:actorcritic})}\strike{We adapt the actor-critic algorithm in [31]} %\cite{yang2019global} 
to find the approximate cost-minimizing controller $K$ for \strike{a given $F$} \azedit{the system $(\bar{A},\bar{B})$}. We consider linear Gaussian feedback policies of the form $\mu_t(X_t) = -K X_t + \zeta_t$ where $K = [K_1, K_2], K_1, K_2 \in \RR^{p \times m}$. This has the structure of the optimal policy $-K X_t$ perturbed by a random term $\zeta_t$ which is generated i.i.d. with distribution $\Ns(0,\sigma^2 I)$ for some $\sigma > 0$. The random term is meant to encourage exploration. {\color{blue}Notice that in the RL setting we use a controller which has closed-loop dependence on the mean-field trajectory. This is not the case when system parameters are known and the MFE can be computed a priori \cite{zaman2020acc}.}
%We use an natural actor-critic algorithm developed in \cite{yang2019global} to 
%obtain an approximate cost-minimizing controller for a mean-field trajectory. 
%Later we obtain convergence guarantees under the general setting where the 
%Markov chain is fast mixing but is not assumed to be fully mixed.

%\aznote{Highlight the non-stationarity. Highlight that our contribution is that we specify the amount of time needed for the critic to converge for an unmixed but fast mixing MC}. 
Each iteration of the actor-critic involves two steps, namely the \emph{actor} and the \emph{critic}. %\strike{ The critic step conducts policy evaluation in a primal-dual manner. The primal variable is denoted by $\hat{\theta}$ and the dual variable  by $\omega$. The variables $\hat\theta$ and $\omega$ are restricted to sets $\Xs_\Theta$ and $\Xs_\Omega$ respectively, which are bounded by constants $R_{\Theta}$ and $R_{\Omega}$.} 
The critic step estimates %\strike{vector  is an estimate of} 
the true parameter vector $\theta := \svec(H_K)$, where matrix $H_K \in \RR^{(2m + p) \times (2m + p)}$ is the $Q$-function parameter matrix. \azedit{ The estimate of the true parameter vector is denoted by $\hat{\theta}$. For the critic we use the GTD policy evaluation method of \cite{yang2019global}. Due to the non-stationary MFE setting of this work, the Markov chain of the system $X_t$ is unmixed but fast mixing. As a result of unmixed Markov chain (as opposed to \cite{yang2019global}), the number of timesteps $T$ (needed to achieve a good estimate by the critic), depends on the initial condition of the system $X_0$. This result is presented in the next section.} \azedit{Once the estimate $\hat\theta$ is obtained} the \emph{actor} step then updates the controller in the direction of the natural policy gradient. %\strike{given the estimate $\hat\theta$}. 
\azedit{After $S$ actor-critic updates we arrive at the approximate cost-minimizing controller for system $(\bar{A},\bar{B})$.}%\strike{Let us define the feature vector at time $t$ to be $\phi_t := \svec \Big( \big(X_t^T, U_t^T \big)^T \big( X_t^T, U_t^T \big) \Big)$. }

%\aznote{This section should give clarification about the information structure, how it is decentralized for the control setting but not for the RL setting. Explain that the the agent’s controller depends on the mean-field trajectory in a closed-loop manner.}
%\aznote{Explain the role of the aggregator.}
\azedit{Once the actor-critic has computed the} approximate cost-minimizing controller $K$ (corresponding to \azedit{$(\bar{A},\bar{B})$}), the \emph{state aggregator} updates the mean-field trajectory $\bar{Z}' = \{ \bar{Z}'_0, \bar{Z}'_1,\ldots \}$. {\color{blue}Essentially the state aggregator simulates the \emph{collective} behavior of infinitely many agents acting under controller $K$. As a result, the learning process is decoupled, since each agent only needs to interact with the aggregator and can disregard the other agents. 
%\strike{which is the aggregate behavior of all agents under the controller $K$}.
An agent under controller $K$ has closed-loop dynamics:}  
\begin{align}\label{eq:state_agg_0}
Z'_{t+1} = (A - B K_1) Z'_t - B K_2 \bar{Z}'_t {\color{blue}+ W'_t}.
\end{align} 
%\strike{Notice this is a closed-loop controller with respect to the agent's state $Z_t$ 
%and mean-field state $\bar{Z}'_t$, in contrast to [ACC paper] where the 
%\emph{mean-field update} uses a controller which is closed-loop in the agent 
%state but is open-loop in the mean-field state.} 
\kznote{what is $W_t'$ here? need to add explanation.}
By aggregating \eqref{eq:state_agg_0}, the updated mean-field trajectory $\bar Z'$ is shown to follow linear dynamics: 
\begin{align} \label{eq:state_agg}
\bar{Z}'_{t+1} = F' \bar{Z}'_t, \text{ where } F' = A - B(K_1 + K_2).
\end{align}
Note that \eqref{eq:state_agg} inherently yields an update rule from $F$ to $F'$ \azedit{(and hence $\bar{A}$ to $\bar{A}'$)}, which parameterizes the updated mean-field trajectory $\bar Z'$. The combination of the actor-critic algorithm for LQG and the \strike{update} \azedit{state aggregator} \eqref{eq:state_agg}, as outlined in Algorithm \ref{alg:actorcritic}, essentially performs an approximate and data-driven update of the operator $\Ts$ (as in \eqref{eq:eq_mf}).
%$\Ts$ (\issue{or $\Ts$??}) defined in the proof of Proposition 
%\ref{lem:exist_unique_linear} (\issue{we need a better echo-back to either the 
%composition of the big $\Xs_\Omega$ and $\Phi$ operator defined before}.), 
\azedit{ If the number of iterations $R$ of the algorithm \ref{alg:actorcritic} are high enough}\strike{which} \azedit{ it converges to the MFE with high probability.} %\emnote{should sounds weak; does it or does it not?}. 
In addition, by Lemma \ref{lem:F_contract}, if the update starts with a \emph{stable} MF state matrix $F \in \FF$, the updated $F'$ is also stable, with high probability. We formally establish these convergence results with finite samples in the next section.

Next, we formally summarize the update rules in Algorithm \ref{alg:actorcritic}. The algorithm consists of an inner and an outer loop. The outer loop iterates over $r \in [R]$ and the inner loop iterates over $s \in [S_r]$. %\emnote{let's index from $1$ and use the [] notation to be consistent with $[N]$} \aznote{Done} 
The inner loop consists of the actor-critic. The critic step observes: 1) the instantaneous rewards $c_t$, 2) the trajectory $X_t$ of the system $(\bar{A}^{(r)},\bar{B})$, where $\bar{A}^{(r)} = \left(\begin{array}{cc}A & 0 \\ 0 & F^{(r)}\end{array} \right)$, and 3) the control actions $U_t$, for $t \in [T_{s,r}]$ time steps. Using this information, the critic step %\emnote{what is ``it''; let's be more clear} 
evaluates the estimate $\hat{\theta}^{(s,r)}$ of the true parameter vector $\theta^{(s,r)}$. This estimate is then used in the actor step to evaluate $K^{(s+1,r)}$ for each $s \in [S_r]$. After $S_r$ iterations, the inner loop outputs $K^{(S_r,r)}$ which yields an approximate cost-minimizing controller for the mean-field trajectory $\bar{Z}^{(r)}$ defined by the mean-field state matrix $F^{(r)}$. Lastly, $K^{(S_r,r)}$ is used by the state aggregator to obtain the next mean-field state matrix $F^{(r+1)}$.


\begin{algorithm}
	\caption{Actor-critic for LQ-MFG} \label{alg:actorcritic}
	\begin{algorithmic}[1]
		\STATE {\bf Input}: Number of iterations: $R$, $\{S_r : r \in [R]\}$, $\{T_{s,r}: s \in [S_r], r \in [R] \}$.
%		\strike{Stepsizes: $\{ \alpha^{(s,r)}_t:t \in [T^{(s,r)}], s \in [S_r], r \in [R] \}$, $\beta$}
		\STATE {\bf Initialize}: $F^{(1)} \in \mathbb{F}$ and stabilizing 
		$K^{(1,1)}$
		\FOR {$r \in [R]$}
			\FOR {$s \in [S_r]$}

				\STATE {\bf Critic Step } Compute $\hat\theta^{(s,r)}$ using GTD for $T_{s,r}$ timesteps\\ %\strike{(Algorithm 2 of [31])} \label{state:critic} \aznote{Remove references of [31] in the algorithm block. Explain the actor and critic step.}
				
				\STATE {\bf Actor Step} Compute $K^{(s+1,r)}$ using $\hat\theta^{(s,r)}$ and $K^{(s,r)}$ %\strike{(Algorithm 1 in [31])}

			\ENDFOR
			
			\STATE {\bf Update mean-field trajectory} $F^{(r+1)}$ using state aggregator and $K^{(S_r,r)}$ \label{state:aggregate} (by \eqref{eq:state_agg})
			
			\STATE $K^{(1,r+1)} \leftarrow K^{(S_r,r)}$
		\ENDFOR
		\STATE {\bf Output}: $K^{(S_R,R)}, F^{(R)}$
	\end{algorithmic}
\end{algorithm}

==> Section4_-_Old.tex <==

We now provide non-asymptotic convergence guarantees for Algorithm \ref{alg:actorcritic}. Moreover, we also provide an error bound for the approximate MFE output, as generated by Algorithm 1, with respect to the NE of the finite population game. %\emnote{no ``finite-agent'' or ``infinite-agent'', write population; check throughout}




\subsection{Non-asymptotic convergence}
We begin by presenting the convergence result of the critic step in the algorithm. The output of this step is the parameter vector estimate $\hat\theta^{(s,r)}$ which is shown to be arbitrarily close to the true parameter vector $\theta^{(s,r)}$ given that the number of time-steps in the critic step $T_{s,r}$ is sufficiently large. 
\begin{proposition} \label{prop:PE}
	For any $r \in [R]$ and $s \in [S_r]$, the parameter vector estimate $\hat{\theta}^{(s,r)}$ satisfies
	\begin{align*}
	\lVert \hat\theta^{(s,r)} - \theta^{(s,r)} \rVert^2_F \leq \kappa^{(s,r)}_1   \frac{ \log^6 T_{s,r} }{\sqrt{T_{s,r}}},
	\end{align*}
	with probability at least $1-T^{-4}_{s,r}$. The variable $\kappa^{(s,r)}_1$ \kznote{what is this variable? do we have an expression for that? I believe I had this comment before. At least in this arxiv version, we do need to show people the expression? how does it depend on the parameters of the problem?} \azedit{is a polynomial of }\strike{depends on} the initial state $X_0$ and controllers $K^{(1,r)}$ and $K^{(s,r)}$.%\kzstrike{what is this $\kappa^{(s,r)}_1$? how large it would be? I think it would be better to give the specific form of it, at least in the arxiv version of this Proposition.} \azstrike{agreed for the ArXiv version}
\end{proposition}
\begin{proof}
	The proof is an adaptation of the technique used in \cite{yang2019global}\strike{ and the reader can refer to it for omitted details}. We provide the main idea of the proof and how it is modified to \strike{cater for} the unmixed \azedit{fast mixing} Markov chain setting. The problem of estimating the parameter vector $\theta^{(s,r)}$ is first formulated as a minimax optimization problem. Then, the estimation error $\lVert \hat\theta^{(s,r)} - \theta^{(s,r)} \rVert^2_F$, is shown to be upper bounded by the duality gap of that minimax problem. Using results from \cite{wang2017finite} an explicit expression is obtained for the duality gap.
	
	Most of the proof from Theorem 4.2 \cite{yang2019global} follows except for two differences: 1) A lower bound on the probability of the event $\Es$ 	in 	equation (5.20) needs to be established, and 2) An upper bound for the 	expression $\EE [\lVert \phi_t \phi^T_{t+1} \hat\theta \rVert^2_2]$, where $\phi_t := \svec \Big( \big(X_t^T, U_t^T \big)^T \big( X_t^T, U_t^T \big) \Big)$, %in equation (5.31) 
	needs to be found. First we lower bound the probability of the event $\Es_{t}$. In the following, we define $T =  T_{s,r}$ for clarity. Let us define the event $\Es$,
	\begin{align*}
	\Es := \bigcap_{t=0}^{T-1}\big\{ \big\lvert \big\lVert X_{t} \big\rVert_2^2 + \big\lVert 	
	U_{t} \big\rVert_2^2 - \EE\big[ \big\lVert X_{t} \big\rVert_2^2 + \big\lVert 
	U_{t} 	\big\rVert_2^2 \big] \big\rvert < C_1 \big\},
	\end{align*} 
	Let us first define an event $\Es_{t}$ such that,
	%\emstrike{replace $i$ with $t$}
	\begin{align*}
	& \Es_{t} := \big\{ \big\lvert \big\lVert X_{t} \big\rVert_2^2 + \big\lVert U_{t} \big\rVert_2^2 - \EE\big[ \big\lVert X_{t} \big\rVert_2^2 + \big\lVert U_{t} \big\rVert_2^2 \big] \big\rvert \geq C_{1,t} \big\},
	\end{align*}
	for some $C_{1,t}>0$ and $t \in \{0,\ldots,T-1\}$. We want to establish an upper bound for the probability $\PP(\Es_{t})$. Suppose $K$ is a stabilizing controller for \eqref{eq:augdynamics} and define $L_K := \bar{A} - \bar{B}K$. Now let us consider control policies of the form $U_{t} = -K X_{t} + \zeta_{t}$ where $\zeta_{t}$ is generated i.i.d. with distribution $\Ns(0,\sigma^2 I)$. The marginal distributions of $X_{t}$ and $U_{t}$ under filtration $\Fs_{0}$ (having observed $X_0$) is,
	\begin{align} \label{eq:X_t}
	X_{t} & \sim \Ns\Big(L_K^{t} X_0, \Sigma_{X,t} \Big), t \in \{0,\ldots,T-1\},\\
	U_{t} & \sim \Ns\Big(K L_K^{t} X_0, K \Sigma_{X,t} K^T + \sigma^2 I 
	\Big), \nonumber
	\end{align}
	where $\Sigma_{X,0} = 0$, $\Sigma_{X,t} = \sum_{s=0}^{t-1} L_K^s \Sigma_X (L_K^s)^T$ for $t \in \{1,\ldots,T-1\}$ \kzstrike{to $T$ or $T-1$.} and $\Sigma_X = \Sigma_{\bar{w}} + \sigma^2 \bar{B} \bar{B}^T$. Let $\tilde{X}_{t} := X_{t} - L_K^{t} X_0$ and $\tilde{U}_{t}:= U_{t} - K L_K^{t} X_0$. By definition $\tilde{X}_{t}$ and $\tilde{U}_{t}$ are zero mean Gaussian random vectors. Now we consider the quantity,
	%	\begin{align} \label{eq:expr_1}
	%	& \big\lVert X_{t} \big\rVert_2^2 + \big\lVert U_{t} 
	%	\big\rVert_2^2 - 
	%	\EE\big[ \big\lVert X_{t} \big\rVert_2^2 + \big\lVert U_{t} 
	%	\big\rVert_2^2 
	%	\big] \nonumber \\
	%	%& = \big\lVert \tilde{X}_{t} + L_K^{t} X_t \big\rVert_2^2 + 
	%	%\big\lVert 
	%	%\tilde{U}
	%	%_{t} + K L_K^{t} X_t \big\rVert_2^2 - \\ 
	%	%& \hspace{1cm} \EE\big[ \big\lVert \tilde{X}_{t} + L_K^{t} X_t 
	%	%\big\rVert_2^2 + \big\lVert \tilde{U}_{t} + K L_K^{t} X_t 
	%	%\big\rVert_2^2 
	%	%\big], \\
	%	& = \big\lVert \tilde{X}_{t} \big\rVert_2^2 + \big\lVert 
	%	\tilde{U}_{t} 
	%	\big\rVert_2^2 - \EE\big[ \big\lVert \tilde{X}_{t} \big\rVert_2^2 + 
	%	\big\lVert 
	%	\tilde{U}_{t} \big\rVert_2^2 \big]  + \nonumber \\
	%	& \hspace{1cm} 2 \big\langle L^{t} X_t, \tilde{X}_{t} \big\rangle + 2 
	%	\big\langle K L^{t} X_t, \tilde{U}_{t} \big\rangle,
	%	\end{align}
	\begin{align} \label{eq:expr_1}
	& \big\lVert X_{t} \big\rVert_2^2 + \big\lVert U_{t} 	\big\rVert_2^2 - \EE\big[ \big\lVert X_{t} \big\rVert_2^2 + \big\lVert U_{t} 	\big\rVert_2^2 	\big] = \big\lVert \tilde{X}_{t} \big\rVert_2^2 + \big\lVert \tilde{U}_{t} 	\big\rVert_2^2 - \nonumber \\
	& \EE\big[ \big\lVert \tilde{X}_{t} \big\rVert_2^2 + \big\lVert \tilde{U}_{t} \big\rVert_2^2 \big]  +  2 	\big\langle L^{t-1} X_t, \tilde{X}_{t} \big\rangle + 2 	\big\langle K L^{t-1} X_t, \tilde{U}_{t} \big\rangle,
	\end{align}
	%The last equality is obtained by the following reasoning. For any $V_1, 
	%V_2 \in 
	%\RR^n$, $\lVert V_1 + V_2 \rVert_2^2 = \langle V_1 + V_2, V_1 + 
	%V_2\rangle$. 
	%Using linearity of the inner product in its first argument and additivity 
	%in 
	%the 
	%second argument we get $\lVert V_1 + V_2 \rVert_2^2 = \lVert V_1\rVert_2^2 
	%+ 
	%\lVert V_2 \rVert_2^2 + 2 \langle V_1, V_2\rangle$. Finally the terms 
	%$\langle 
	%L^{t} X_1, \tilde{X}_{t} \rangle$ and $\langle K L^{t} X_1, 
	%\tilde{U}_{t} \rangle$ are zero mean Gaussian variables due to the 
	%fact 
	%that they are linear combinations of zero mean Gaussian vectors. 
	Let $V_{t} = [\tilde{X}^T_{t}, \tilde{U}^T_{t}]^T$ which, using \eqref{eq:X_t} and the definition of $V_{t}$, has the distribution $\Ns(0,\Sigma^{t}_v)$, where
	\begin{align*}
	%\Sigma^{t}_v & = 
	%\Bigg(\begin{array}{cc}
	%0 & 0 \\
	%0 & \sigma^2 I
	%\end{array} \Bigg) + 
	%\Bigg(\begin{array}{c}
	%I \\
	%-K 
	%\end{array} \Bigg) \Sigma_{X,t}
	%\Bigg(\begin{array}{c}
	%I \\
	%-K 
	%\end{array} \Bigg)^T
	%\\
	\Sigma^{t}_v & = \Bigg(\begin{array}{cc}
	\Sigma_{X,t} & -\Sigma_{X,t} K^T \\
	-K \Sigma_{X,t} &  K \Sigma_{X,t} K^T + \sigma^2 I
	\end{array} \Bigg),
	\end{align*}
	Using the definition of $\Sigma_{X,t}$ we deduce
	\begin{align*}
	\Sigma^{t+1}_v -  \Sigma^{t}_v = \Bigg(\begin{array}{c}
	I \\
	-K 
	\end{array} \Bigg) L^{t}_K \Sigma_X (L^{t}_K)^T
	\Bigg(\begin{array}{c}
	I \\
	-K 
	\end{array} \Bigg)^T ,
	\end{align*}
	which means $\Sigma^{t+1}_v \geq \Sigma^{t}_v$. Moreover, for a stabilizing $K$, $X_{t}$ and consequently $V_t$ converges to a stationary distribution as $t \rightarrow \infty$. Let us denote the covariance of this distribution by $\Sigma_v^{\infty}$. And since $\Sigma^{t+1}_v \geq \Sigma^{t}_v \implies \Sigma^{\infty}_v \geq \Sigma^{t}_v$. Using $V_{t}$ the expression in \eqref{eq:expr_1} can be written as,
	\begin{align*}
	& \lVert X_{t} \rVert_2^2 + \lVert U_{t} \rVert_2^2 - \EE\big[ \lVert X_{t} \rVert_2^2 + \lVert U_{t} \rVert_2^2 \big] \\
	& = \lVert V_{t} \rVert_2^2 - \EE \big[ \lVert V_{t} \rVert_2^2 \big] + \underbrace{2 \Big\langle \Big[\begin{array}{c} L^{t} X_0 \\ K L^{t} X_0 \end{array}\Big], V_{t} \Big\rangle}_{v_{t}}.
	\end{align*}
	By definition $v_{t}$ has the distribution $\Ns (0, \sigma_v^t )$ where
	\begin{align*}
	\sigma_v^t = 4\bigg[\begin{array}{c} L^{t} X_0 \\ K L^{t} X_0 \end{array}\bigg]^T \Sigma^{t}_v \bigg[\begin{array}{c} L^{t} X_0 \\ K 	L^{t} X_0 \end{array}\bigg].
	\end{align*}
	This is upper bounded by,
	\begin{align}
	\sigma_v^t & \leq 4(1+\lVert K \rVert^2_F) \lVert\Sigma^{t}_v \rVert_2 \lVert X_0 \rVert^2_2 \nonumber\\
	& \leq 4(1+\lVert K \rVert^2_F) \lVert\Sigma^{\infty}_v \rVert_2 \lVert X_0 
	\rVert^2_2 := \sigma^{\infty}_v.
	\end{align}
	Now let us define events $\Es^1_{t}$, $\Es^2_{t}$, 
	$\Es^3_{t}$ 
	and 
	$\Es^4_{t}$ for $t \in \{0,\ldots,T-1\}$ \kzstrike{previously in the proof you had $0,\cdots, T-1$, right now have $[T]$. are they consistent? check all plz.} such that
	\begin{align*}
	& \Es^1_{t} := \big\{ \big\lvert \lVert V_{t} \rVert_2^2 - \EE \big[ \lVert V_{t} \rVert_2^2 \big] \big\rvert +  \big\lvert v_{t} \big\rvert \geq C_{1,t} \big\}, \\
	& \Es^2_{t} := \big\{ \big\lvert  \lVert V_{t} \rVert_2^2 - \EE \big[ \lVert V_{t} \rVert_2^2 \big] \big\lvert < C_{2,t} \,\,\, \& \,\,\, \big\lvert v_{t} \big\rvert < C_3 \big\},  \\
	& \Es^3_{t} := \big\{ \big\lvert  \lVert V_{t} \rVert_2^2 - \EE \big[ \lVert V_{t} \rVert_2^2 \big] \big\lvert \geq C_{2,t} \big\}, \hspace{0.25cm}\Es^4_{t} := \big\{ \big\lvert v_{t} \big\rvert \geq C_3 \big\},
	\end{align*}
	where $C_{2,t} , C_3 > 0$ and $C_{1,t} = C_{2,t} + C_3$. From triangle 
	inequality, we have
	\begin{align*}
	\big\lvert \lVert V_{t} \rVert_2^2 - \EE \big[ \lVert V_{t} 	\rVert_2^2 	\big] + v_{t} \big\rvert \leq \big\lvert \lVert V_{t} \rVert_2^2 - \EE \big[ \lVert 	V_{t} 	\rVert_2^2 \big] \big\rvert + \big\lvert v_{t} \big\rvert
	\end{align*}
	and therefore $\Es_{t} \subset \Es^1_{t}$. Moreover, $\Es^1_{t} \cap \Es^2_{t} = 	\varnothing \implies \Es^1_{t} \subset \big(\Es^2_{t} \big)^c \implies 	\Es_{t} \subset \big(\Es^2_{t} \big)^c = \Es^3_{t} \cup \Es^4_{t}$, and hence
	\begin{align} \label{eq:upper_bound_events}
	%	&\Es^1_{t} \cap \Es^2_{t} = \varnothing \implies 
	%	\Es^1_{t} 
	%	\subset \big(\Es^2_{t} \big)^c \nonumber\\ 
	%	&\implies \Es_{t} \subset \big(\Es^2_{t} \big)^c = \Es^3_{t} 
	%	\cup 
	%	\Es^4_{t}, \nonumber \\
	\PP(\Es_{t}) \leq \PP(\Es^3_{t} \cup \Es^4_{t}) \leq \PP(\Es^3_{t}) + 
	\PP(\Es^4_{t}).
	\end{align} 
	First we establish an upper bound for $\PP (\Es^3_{t})$ for $t \in \{0,\ldots,T-1\}$\kzstrike{see comments above. be consistent.}. Using Hanson-Wright inequality \cite{rudelson2013hanson},
		\begin{align} \label{eq:P_eps_3}
		\PP(\Es^3_{t}) \leq 2   e^{-C   \min \big((C_{2,t})^2   \lVert 
			\Sigma^{t}_v \rVert_F^{-2}, C_{2,t}   \lVert \Sigma^{t}_v 
			\rVert^{-1}_2 \big)},
		\end{align}
		for a $C>0$. Substituting $C_{2,t} = k_1 \log(T/3) \lVert \Sigma^{t}_v \rVert_2$ for any $k_1 \geq \max(6/C, (p+2m) (\log (T/3))^{-1})$ using a method similar to \cite{yang2019global} we get
		\begin{align} \label{eq:P_eps_3_1}
		& (C_{2,t})^2   \lVert \Sigma^{t}_v \rVert_F^{-2} = k^2_1   (\log (T/3))^2 \lVert \Sigma^{t}_v \rVert_2^2   \lVert \Sigma^{t}_v \rVert_F^{-2} \geq \\
		&  k^2_1   (\log (T/3))^2   (p+2m)^{-1} \geq k_1   \log (T/3) =  C_{2,t} \lVert \Sigma^{t}_v \rVert^{-1}_2. \nonumber
		\end{align}
		The first inequality is due to the relation between the induced and 
		Frobenius norms and the second inequality is due to definition of $k_1$. Using equations \eqref{eq:P_eps_3}, \eqref{eq:P_eps_3_1} and the expression for $C_{2,t}$ \kzstrike{why the following equation starts with no sentence?}
		\begin{align} \label{eq:P_eps_1}
		\PP(\Es^3_{t}) \leq \frac{2 T^{-C   k_1}}{3} \leq \frac{2 T^{-6}}{3},
		\end{align}
	where $C$ is an absolute constant. Now we establish an upper bound for $\PP(\Es^4_{t})$ using Gaussian 
	tail bounds \kzstrike{what is ``Gaussian concentration bounds''? any reference? do you mean Gaussian tail bounds? plz be careful and check the reference, before using any term.}, $\PP(\Es^4_{t}) \leq 2 e^{ -C^2_3/(2\sigma_v^t) }.$
	Substituting $C_3 = k_2   \log (T/6)   \sqrt{2\sigma^{\infty}_v}$ and choosing $k_2 \geq \max (6,(\log (T/6))^{-1})$, we get
	\begin{align}  \label{eq:P_eps_2}
	\PP(\Es^4_{t}) \leq \frac{T^{-k_2}}{3} \leq \frac{T^{-6}}{3}.
	\end{align}
	The first inequality is due to $\frac{C^2_3}{2\sigma_v^t} \geq k_2^2 (\log (T/6))^2 \geq k_2 \log (T/6)$. Now using \eqref{eq:upper_bound_events}, 
	\eqref{eq:P_eps_1} 
	and \eqref{eq:P_eps_2}, we deduce
	\begin{align}
	\PP(\Es_{t}) \leq T^{-6}.
	\end{align}
	%	Finally we establish upper bound on $C_{1,t}$ that does not depend on $t$,
	Finally we obtain a time invariant upper bound on $C_{1,t}$:
	\begin{align}
	C_{1,t} & = C_{2,t} + C_3  \\%=k_1 \log(T/3) \lVert \Sigma^{t}_v \rVert_2 + k_2   \log (T/6)   \sqrt{2\sigma^{\infty}_v} \nonumber \\
	& \leq k_1 \log(T/3) \lVert \Sigma^{\infty}_v \rVert_2 + k_2 \log (T/6) \sqrt{2\sigma^{\infty}_v} =: C_1 . \nonumber
	\end{align}
	Let us define another event,
	\begin{align*}
	\Es^*_{t} := \big\{ \big\lvert \big\lVert X_{t} \big\rVert_2^2 
	+ 
	\big\lVert U_{t} \big\rVert_2^2- \EE\big[ \big\lVert X_{t} \big\rVert_2^2 + 
	\big\lVert 
	U_{t} 
	\big\rVert_2^2 \big] \big\rvert \geq C_1 \big\}.
	\end{align*}
	Since $C_1 \geq C_{1,t}$, $\Es^*_{t} \subset \Es_{t} \implies 
	\PP(\Es^*_{t}) \leq P(\Es_{t}) \leq T^{-6}$. Moreover, $\PP(\cup_{i=0}^{T-1} \Es^*_{t} ) \leq \sum_{i=0}^{T-1} \PP(\Es^*_{t}) \leq T^{-5}$.\emstrike{check limits $T$ or $T-1$? check throughout}\kzstrike{nice catch. I had comments/concerns above, too. plz check all.} Now we can bound 
	\begin{align*}
	\PP(\Es) = 1 - \PP(\cup_{i=0}^{T-1} \Es^*_{t}) \geq 1 - T^{-5} .
	\end{align*}
	Now we bound the expression $\EE [\lVert \phi_t \phi^T_{t+1} 
	\hat\theta \rVert^2_2]$ in equation (5.31). in \cite{yang2019global}:
	\begin{align} \label{eq:bound_quant}
	& \EE [\lVert \phi_t \phi^T_{t+1} \hat\theta \rVert^2_2] = \EE [\hat\theta^T 
	\phi_{t+1} 	\phi^T_t \phi_t \phi^T_{t+1} \hat\theta]  \nonumber \\ 
	& = \EE [\phi^T_t \phi_t \hat\theta^T \phi_{t+1} \phi^T_{t+1} 
	\hat\theta] \leq \EE \big[\phi^T_t \phi_t  \big] \lVert \hat\theta 
	\rVert^2_2 \EE 
	\big[ \lVert \phi_{t+1} \phi^T_{t+1} \rVert_2 \big] \nonumber \\
	& \leq \EE \big[ \phi^T_t \phi_t  \big] 
	\lVert \hat\theta \rVert^2_2 \EE \big[ \lVert \phi_{t+1} \phi^T_{t+1} 
	\rVert_F 
	\big] \nonumber\\
	& \leq \EE \big[ \phi^T_t \phi_t  \big] \lVert \hat\theta \rVert^2_2 \EE 
	\big[ 
	\lVert \phi_{t+1} \rVert^2_F \big] \nonumber\\
	& = \EE \big[ \phi^T_t \phi_t  \big] \lVert \hat\theta \rVert^2_2 \EE \big[ 
	\tr(\phi_{t+1} \phi^T_{t+1} )\big] \nonumber\\ 
	& = \EE \big[ \phi^T_t \phi_t  \big] \lVert \hat\theta \rVert^2_2 \EE \big[ 
	\phi^T_{t+1} \phi_{t+1}\big].
	\end{align}
	The first inequality is due to the Cauchy-Schwarz inequality. Using the 
	definition of $\phi_t$,
	%\begin{align*} 
	$\phi^T_t \phi_t = %\\
	%& \svec \left( \left( \begin{array}{c}
	%X_t \\ U_t
	%\end{array} \right) \left( \begin{array}{c}
	%X_t \\ U_t
	%\end{array} \right)^T \right)^T \svec \left( \left( \begin{array}{c}
	%X_t \\ U_t
	%\end{array} \right) \left( \begin{array}{c}
	%X_t \\ U_t
	%\end{array} \right)^T \right) \\
	%& = \left( \begin{array}{c}
	%X_t \\ U_t
	%\end{array} \right)^T \left( \begin{array}{c}
	%X_t \\ U_t
	%\end{array} \right) \left( \begin{array}{c}
	%X_t \\ U_t
	%\end{array} \right)^T \left( \begin{array}{c}
	%X_t \\ U_t
	%\end{array} \right)
	\big\lVert \big( X_t^T, U_t^T \big)^T \big\rVert^4_2$. 
	%\end{align*}
	Hence an upper bound for the expectations on the RHS of \eqref{eq:bound_quant} can be obtained by using the fourth moments of the marginal distributions of $X_t$ and $U_t$ given in \eqref{eq:X_t}. Hence the bound on $\EE [\lVert \phi_t \phi^T_{t+1} \hat\theta \rVert^2_2]$ would be a function of the initial state $\lVert X_1 \rVert_2$, the stationary distribution $\Sigma_v^{\infty}$ and $\sigma^{\infty}_v$, and the bound on $\lVert \hat\theta \rVert^2_2$, imposed by the critic \cite{yang2019global} using a projection operator.
\end{proof}

%\begin{blockremove}
%\begin{proposition} \label{prop:PE}
%For $T_{s,r}$ sufficiently large %\emnote{can we quantify more?}\aznote{carry-over from \cite{yang2019global}} 
%and stepsizes $\alpha^{\omt{(s,r)}}_t = \alpha/\sqrt{t}$, the parameter vector $\hat{\theta}^{(s,r)}$ in Algorithm \ref{alg:actorcritic} satisfies
%\begin{align*}
%\lVert \hat\theta^{(s,r)} - \theta^{(s,r)} \rVert^2_F \leq \frac{\Upsilon_1}{\omt{(1-\rho) (\kappa_{K^{(s,r)}})^2 }}   \frac{ \log^6 T_{s,r} }{\sqrt{T_{s,r}}},
%\end{align*}
%with probability at least $1-T^{-4}_{s,r}$. %In the expression $
%%\theta_{K^{(s,r)}}$ is the 
%%parameter vector for the 
%%$Q$ function corresponding to feedback matrix $K^{(s,r)}$ and 
%The constant $\omt\rho$ lies in the interval $\omt{(\rho(\bar{A}^{(r)} - \bar{B} K^{(s,r)}) , 1)}$ and $\Upsilon_1$ depends on $X_0, \omt {R_{\Theta}}, \omt{R_{\Omega}}, \omt{J(K^{(1,r)})}, \omt{\lVert K^{(s,r)}\rVert_F}$ and $ \omt{\sigma_{\min}(C_X)}$.%\emnote{original text made it seem like $\rho$ also depended on the listed quantities}
%\end{proposition}
%\end{blockremove}
%\begin{proof}[Proof Sketch]
%%\kzstrike{I would call it a ``proof sketch''? Also, since currently we will have an arxiv version (with no space limitation), I think you do need a ``complete'' proof there, and refer to it from here, saying that we only include a sketch here.}
%%\strike{Most of the proof carries over from Theorem 4.2 of [31], except for an upper bound on the probability of the event $\Es$ in (5.20) and an upper bound for $\EE [\lVert \phi_t \phi^T_{t+1} \hat\theta \rVert^2_2]$ in (5.31).} 
%The proof is an adaptation of the technique used in \cite{yang2019global} and the reader can refer to it for omitted details. We provide the main idea of the proof and how it is modified to cater for the unmixed MC setting. The problem of estimating the parameter vector $\theta^{(s,r)}$ is first formulated as a minimax optimization problem. Then the estimation error, $\lVert \hat\theta^{(s,r)} - \theta^{(s,r)} \rVert^2_F$, is shown to be upper bounded by the duality gap of that minimax problem. Using results from \cite{wang2017finite} an explicit expression is obtained for the duality gap.
%%\aznote{Provide general idea of proof and how it is modified for the current setting}
%%\strike{Most of the proof from Theorem 4.2 {yang2019global} follows except for two instances. 1) An upper bound on the probability of the event $\Es$ in equation (5.20) needs to be established, and 2) An second, an upper bound for the expression $\EE [\lVert \phi_t \phi^T_{t+1} \hat\theta \rVert^2_2]$ in equation (5.31) needs to be found.} These differences are due to the fact that the Markov chain is not assumed to be fully mixed. 
%
%The technique used in \cite{yang2019global} to prove convergence of the critic, assumes that $X_t$ and $U_t$ are bounded. Towards that end consider the event, %\kzstrike{the reasoning for this sentence is not clear to me} %\emnote{use bigcap instead of cap for indexed operators; check throughout}
%$
%\Es := \bigcap_{t=0}^{T-1} \big\{ \big\lvert \big\lVert X_{t} \big\rVert_2^2 + \big\lVert U_{t} \big\rVert_2^2 - \EE\big[\big\lVert X_{t} \big\rVert_2^2 + \big\lVert U_{t} 	\big\rVert_2^2 \big] \big\rvert < C_1 \big\},
%$
%where $T = T_{s,r}$. We will obtain a lower bound for the probability $\PP(\Es)$. This lower bound will contribute to the probabilistic guarantees of the lemma. To that end, let us first define an event
%$
%\Es_{t} := \big\{ \big\lvert \big\lVert X_{t} \big\rVert_2^2 + \big\lVert U_{t} \big\rVert_2^2 - \EE\big[ \big\lVert X_{t} \big\rVert_2^2 + \big\lVert U_{t} \big\rVert_2^2 \big] \big\rvert \geq C_{1,t} \big\},
%$
%%for some $C_{1,t}>0$ and 
%for $t \in \{0,\ldots,T-1\}$. Due to the fact that the MC is not mixed, the random vectors $X_t$ and $U_t$ have non-zero mean, non-stationary marginal distributions. %\kzstrike{I have trouble understanding this sentence. Even if the  chain mixes, $\lVert X_{t} \rVert_2^2 + \lVert U_{t} \rVert_2^2$ is always non-negative and the mean is NEVER zero, right??}. 
%This is opposed to the mixed MC setting of  \cite{yang2019global}, which leads to $X_t$ and $U_t$ having zero mean and stationary marginal distributions. Hence we develop a method to lower bound $\PP(\Es)$ in the unmixed MC setting. {Towards that end we first define quantities, $V_t$ and $v_t$ such that $V_{t} = [(X_{t} - L_K^{t} X_0)^T, (U_{t} - K L_K^{t} X_0)^T]^T$ and $v_t = 2 \Big\langle \Big[\begin{array}{c} L^{t}_K X_0 \\ K L^{t}_K X_0 \end{array}\Big], V_{t} \Big\rangle$, where $L_K = A - B K$ and $K$ is a stabilizing controller. % and $U_{t} = -K X_{t} + \zeta_{t}$ as stated in Section \ref{sec:RL}. 
%As a result of the definition, $V_t$ and $v_t$ are zero mean Gaussian variables and $\lVert X_{t} \rVert_2^2 + \lVert U_{t} \rVert_2^2 = \lVert V_{t} \rVert_2^2 + v_t$. The stationary distributions of $V_t$ and $v_t$ are denoted by $\Ns(0,\Sigma^{\infty}_v)$ and $\Ns (0, \sigma_v^{\infty} )$ and are conditional on $X_0$. %and can be calculated by using the marginal distribution of $X_t$ and $U_t$ conditional on the filtration at time $t=0$, denoted by $\Fs_{0}$. 
%We define two events to bound the concentration of $\lVert V_{t} \rVert_2^2$ and $\big\lvert v_{t} \big\rvert$  separately:
%$\Es^*_{t} := \big\{ \big\lvert  \lVert V_{t} \rVert_2^2 - \EE \big[ \lVert V_{t} \rVert_2^2 \big] \big\lvert \geq C_{2,t} \big\}, \hspace{0.25cm}\Es'_{t} := \big\{ \big\lvert v_{t} \big\rvert \geq C_3 \big\}
%$. The probability $\PP(\Es^*_{t})$ can be upper bounded by using Hanson-Wright inequality and $\PP(\Es'_{t})$ by using Gaussian concentration bounds. Using these bounds we can deduce the upper bound on $\PP(\Es_{t})$ and using a union bound type argument lower bound $\PP(\Es)$. This bound will depend on $\lVert X_0 \rVert_2$ as a result of the MC $X_t, U_t$ being unmixed.}
%%{\color{gray}We begin by defining marginal distributions for this quantity, under any stabilizing control $U_{t} = -K X_{t} + \zeta_{t}$ %(where $\zeta_{t}$ is generated i.i.d. with distribution $\Ns(0,\sigma^2 I)$), 
%%conditional on the filtration at time $t=0$, denoted by $\Fs_{0}$.
%%\vspace{-0.1cm}\begin{align} \label{eq:X_t_U_t_marg}
%%X_{t} & \sim \Ns\Big(L_K^{t} X_0, \Sigma_{X,t} \Big),\\
%%U_{t} & \sim \Ns\Big(K L_K^{t} X_0, K \Sigma_{X,t} K^T + \sigma^2 I 
%%\Big), \nonumber \vspace{-0.15cm}
%%\end{align}
%%where $\Sigma_{X,t} = \sum_{s=0}^{t} L_K^s \Sigma_X (L_K^s)^T$ and $\Sigma_X = \Sigma_{\bar{w}} + \sigma^2 \bar{B} \bar{B}^T$. We notice that the marginal distribution of $X_t, U_t$ is dependent on $\lVert X_0 \rVert_2$. As a result the bounds we obtain will depend on $\lVert X_0 \rVert_2$. Next we split up the quantity $\lVert X_{t} \rVert_2^2 + \lVert U_{t} \rVert_2^2$ using $V_t$ and $v_t$ where $V_{t} = [(X_{t} - L_K^{t} X_0)^T, (U_{t} - K L_K^{t} X_0)^T]^T$ and $v_t = 2 \Big\langle \Big[\begin{array}{c} L^{t}_K X_0 \\ K L^{t}_K X_0 \end{array}\Big], V_{t} \Big\rangle$. The distributions of $V_t$ and $v_t$ are $\Ns(0,\Sigma^{t}_v)$ and $\Ns (0, \sigma_v^t )$, respectively. Due to $K$ being a stabilizing controller, $V_t$ and $v_t$ also have stationary distributions given by $\Ns(0,\Sigma^{\infty}_v)$ and $\Ns (0, \sigma_v^{\infty} )$, respectively. Using these terms, $\lVert X_{t} \rVert_2^2 + \lVert U_{t} \rVert_2^2 = \lVert V_{t} \rVert_2^2 + v_t$. Next we define two events to bound the concentration of $V_t$ and $v_t$ separately:
%%\begin{align*}
%%\Es^*_{t} := \big\{ \big\lvert  \lVert V_{t} \rVert_2^2 - \EE \big[ \lVert V_{t} \rVert_2^2 \big] \big\lvert \geq C_{2,t} \big\}, \hspace{0.25cm}\Es'_{t} := \big\{ \big\lvert v_{t} \big\rvert \geq C_3 \big\}
%%\end{align*}
%%where $C_{1,t} = C_{2,t} + C_3$. Substituting $C_{2,t} = k_1 \log(2 T/3) \lVert \Sigma^{t}_v \rVert_2$ for any $k_1 \geq \max(6/C, (p+2m) (\log (2T/3))^{-1})$ using Hanson-Wright inequality in a method similar to \cite{yang2019global} we get, $\PP(\Es^*_{t}) \leq 4 T^{-6}/3$. Similarly substituting $C_3 = k_2 \log (2T/3) \sqrt{2\sigma^{\infty}_v}$, choosing $k_2 \geq \max (6,(\log (2T/3))^{-1})$ and using Gaussian concentration bounds, $\PP(\Es'_{t}) \leq 2T^{-6}/3$. From these concentration bounds we can deduce $\PP(\Es_{t}) \leq 2 T^{-6}$. Finally by defining $C_1 := \big( k_1 \lVert \Sigma^{\infty}_v \rVert_2 + k_2 \sqrt{2\sigma^{\infty}_v} \big) \log T$, we can conclude that $\PP(\Es) \geq 1 - 2 T^{-5}$.}
%%{\color{gray}We split the term $\big\lVert X_{t} \big\rVert_2^2 + \big\lVert U_{t} \big\rVert_2^2$ into two terms. The first one is a square of a zero-
%%mean Gaussian RV and hence it can be bounded by using Hansen-Wright inequality. The second one is a zero-mean Gaussian RV and is bounded by using Gaussian concentration bounds. These bounds are time varying so finally we obtain time invariant bounds using stationary distribution induced by controller $K^{(s,r)}$.}
%%Now we upper bound the LHS of equation (5.31) in \cite{yang2019global}. Using Cauchy-Schwarz inequality and matrix manipulations, $\EE [\lVert \phi_t \phi^T_{t+1} \hat\theta \rVert^2_2] \leq \EE \big[ \phi^T_t \phi_t \big] \lVert \hat\theta \rVert^2_2 \EE \big[ \phi^T_{t+1} \phi_{t+1}\big]$. Furthermore, $\phi^T_t \phi_t = \big\lVert \big( X_t^T, U_t^T \big)^T \big\rVert^4_2$, which can be bounded by using the fourth moments of the marginal distributions of $X_t$ and $U_t$ which will depend on $\lVert X_0 \rVert_2$.% given in \eqref{eq:X_t_U_t_marg}.
%\end{proof}

Note that in Proposition \ref{prop:PE}, %\strike{is cite{yang2019global} but with one key difference. In our case, $\Upsilon_1$} 
$\kappa^{(s,r)}_1$ \azedit{is a polynomial of} \azstrike{explicitly depends on} \kzstrike{where is it?? which equation is the expression?} the initial state, $X_0$. %\strike{(before start of the critic step)} 
%\kzstrike{How? This constant is too abstract here...}\azstrike{Let us keep it abstract for the camera-ready version}. 
This dependence is due to the MC not being fully mixed. Following the techniques in proof of Theorem 4.2 in \cite{yang2019global}, \strike{$\kappa^{(s,r)}_1$ can be shown to be a monotonically increasing function of $\lVert X_0 \rVert_2$}. \azstrike{If everything else is held constant and only $X_0$ is allowed to change then, $\kappa^{(s,r)}_1 = \Os(\lVert X_0 \rVert_2^4)$. You guys can suggest how to say this.}\kzstrike{where is the expression?? how can people see the dependence?} Having proved a finite\kzedit{-}sample bound on the estimation error for the critic step, %\strike{the policy gradient in the actor step in Algorithm ref{alg:actorcritic} is close to the true natural policy gradient cite{yang2019global}.} 
we now state the convergence guarantee for the actor-critic algorithm for fixed mean-field trajectory. In particular, the approximate cost-minimizing controller found by the actor-critic $K^{(S_r,r)}$, can be brought arbitrarily close to the cost-minimizing controller $K^{(*,r)}$, by choosing the number of iterations of critic, $T_{s,r}$, and actor-critic, $S_r$, sufficiently large. %\strike{Thus, the actor critic algorithm should converge to the cost-minimizing controller approximately, as shown next.}
\begin{proposition} \label{prop:RL-LQG}
	For any $r \in [R]$, let $K^{(1,r)}$ be a stabilizing controller and $S_r$ be chosen such that $S_r \geq  \kappa_2 \lVert \Sigma_{K^{(*,r)}} \rVert_2 \log\big( 2\big(J(K^{(1,r)},F^{(r)}) - J(K^{(*,r)},F^{(r)})\big) / \epsilon_r \big)$, 
	for any $\epsilon_r > 0$, where $\Sigma_{K^{(*,r)}}$ is the covariance matrix of stationary distribution induced by controller $K^{(*,r)}$. Moreover, let $T_{s,r} \geq (\kappa^{(s,r)}_1)^{5/2} \epsilon^{-5}_r$ for $s \in S_r$. Then, with probability at least $1 - \epsilon^{10}_r$,
	\begin{align*}
	& J(K^{(S_r,r)},F^{(r)}) - J(K^{(*,r)},F^{(r)}) \leq \epsilon_r, \\
	& \hspace{0.9cm} \lVert K^{(S_r,r)} - K^{(*,r)} \rVert_F \leq \sqrt{ \kappa_3 \epsilon_r },
	\end{align*}
	and $K^{(s,r)}$ are stabilizing for $s \in S_r$. The variable $\kappa^{(s,r)}_1$ \kzstrike{same here, where is this defined?} is dependent on $K^{(1,r)}, K^{(s,r)}$ and initial state $X_0$ (as in Proposition \ref{prop:PE}). The parameter $\kappa_2$ is an absolute constant and $\kappa_3 = \lVert \Sigma_{w} + \sigma^2 B B^T \rVert_2^{-1} \lVert C_U \rVert_2^{-1}$. \kznote{why did u only write out $\kappa_3$, not $\kappa_2$?}\aznote{$\kappa_2$ is taking verbatim from Zhouran paper.}
\end{proposition}
%\begin{blockremove}
%\begin{proposition} \label{prop:RL-LQG}
%If $K^{(1,r)}$ is a stabilizing controller for system $(\bar{A}^{(r)},\bar{B})$, set the stepsize $\omt{\beta = \lVert C_U \rVert + \sigma^{-1}_{\min}(\Sigma_{\bar{w}}) \big\lVert \bar{B} \big\rVert^2 J \big(K^{(1,r)} \big)} $ and perform $S_r$ updates in the actor-critic algorithm, where 
%\begin{align*}
%S_r \geq C \big\lVert \Sigma_{K^{(*,r)}} \big\rVert \log\big( \omt{2 J(K^{(1,r)} \big) - 2J \big(K^{(*,r)} \big)} / \epsilon_r \big) /\beta,
%\end{align*}
%for any sufficiently small $\epsilon_r > 0$. Furthermore, if at each iteration $r$ we set the number of iterations $T_{s,r}$ to be
%\begin{align*}
%T_{s,r} \geq \omt{\Upsilon_2 \big(\kappa_{K^{(s,r)}} \big)^{-5} \big(1 - \rho \big(L_{K^{(s,r)}} \big)\big)^{-5/2}} \epsilon^{-5}_r,
%\end{align*}
%where $\Upsilon_2$ depends on $J(K^{(1,r)})$ and $\lVert K^{(s,r)}\rVert_F$, then, with probability at least $1 - \epsilon^{10}_r$,
%\begin{align*}
%& \hspace{0.5cm} J(K^{(S_r,r)},F^{(r)}) - J(K^{(*,r)},F^{(r)}) \leq \epsilon_r, 
%\\ & \lVert K^{(S_r,r)} - K^{(*,r)} \rVert_F \leq \sqrt{ \omt {\sigma_{\min}^{-1}(\Sigma_X) \sigma_{\min}^{-1}(C_U)} \epsilon_r },
%\end{align*}
%and {$K^{(S_r,r)}$ is a stabilizing controller }and $K^{(*,r)}$ is the cost-minimizing controller for the system $(\bar{A}^{(r)},\bar{B})$.% and $\Sigma_X = \Sigma_{\bar{w}} + \sigma^2 \bar{B}\bar{B}^T$.
%\end{proposition}
%\end{blockremove}
The first inequality and the stability guarantee in Proposition \ref{prop:RL-LQG} follows from Theorem 4.3 in \cite{yang2019global} and the second inequality can be obtained from proof of Lemma D.4 in \cite{fu2019actor}. 
%\kzstrike{I have question on this Proposition. Where does $\kappa^{(s,r)}_1$ play a role? Since you said your critic is different from cite{fu2019actor}, why doesn't the results from critic appear here? The Proposition 3's proof is not proving anything...} \azstrike{I believe $\kappa_1$ and $\kappa_2$ should be linked in some way, I will figure out and get back.}\kzstrike{please do.} \azstrike{The variable previously denoted by $\kappa^{(s,r)}_2 = (\kappa^{(s,r)}_1)^{5/2}$. So I changed it in the statement of Prop 3 and renamed the other variables.}
Next, we provide the non-asymptotic convergence guarantee %\strike{of the outer-loop of} 
for Algorithm \ref{alg:actorcritic}. We prove that the output of Algorithm \ref{alg:actorcritic}, also called the \emph{approximate} MFE $(K^{(S_R,R)}, F^{(R)})$, approaches the MFE of the LQ-MFG $(K^*, F^*)$. We also provide an upper bound on the difference in cost $J$ under the approximate and the  exact MFE.%\kzstrike{This sentence does not read well to me.. what is the ``bounds on increase''?}\azstrike{rewritten}\kzstrike{I  re-wrote again.} \azstrike{Looks better now}

\begin{theorem} \label{thm:conv_guarantee}
	For any $r \in [R]$, let $\epsilon_r$ be defined as
	\begin{align}
	& \epsilon_r = \kappa_3^{-1} \min \Bigg( \frac{\epsilon^2}{2^{2r+4} \lVert B \rVert_2^2}, \frac{\epsilon^2}{2}, \frac{(1-T_P)^2}{ 8 \lVert B \rVert_2^2} \Bigg) ,
	\end{align}
	and the number of iterations $R$ satisfy,
	$R \geq \log \big( 2\lVert F^{(1)} - F^* \rVert_2 \epsilon^{-1} \big) / \log(1/T_P)$, \azedit{(where $T_P$ is defined in Assumption \ref{asm:boundforcontract}) and }\kzstrike{what is this $T_P$? recall it.}
	\strike{for any} $\epsilon > 0$. Then, with probability at least $1 - \epsilon^5$, $F^{(r)} \in \FF$, $K^{(1,r)}$ is stabilizing for $r \in [R]$, and
	\begin{align*}
	& \lVert F^{(R)} - F^* \rVert_2 \leq \epsilon, \lVert K^{(S_R,R)} - K^* \rVert_2 \leq (1 + D_0 ) \epsilon, \\
	& \hspace{0.8cm} J(K^{(S_R,R)},F^{(R)}) - J(K^*,F^*) \leq D_1 \epsilon ,
	\end{align*}
	where $D_0$, $D_1$ are absolute constants. 
\end{theorem}

%\begin{blockremove}
%\begin{theorem} \label{thm:conv_guarantee}
%For any $\epsilon > 0$ such that $\epsilon < \bar{\epsilon} \omt{:= \sqrt[6]{\log(1/T_P)/(2 \lVert F^{(1)} - F^*\rVert_2)}}$, if the number of iterations $R = \Os(\epsilon^{-5})$ such that,
%\begin{align*}
%R \geq \log \big( \omt{2\lVert F^{(1)} - F^* \rVert_2} \epsilon^{-1} 
%\big) / \omt{\log(1/T_P)} ,
%\end{align*}
%and for each $1 \leq r \leq R$, defining $\epsilon_r$ such that,
%\begin{align} \label{eq:epsilon_s}
%& \epsilon_r = \omt{\sigma_{\min}(\Sigma_X) \sigma_{\min}(C_U)} \min \Big( \epsilon^2  
%/ \big( 2^{2r+4} \lVert B \rVert_2^2 \big), \epsilon^2 /2, \nonumber \\
%& \hspace{4cm} (1-T_P)^2 / \big( 8 \lVert B \rVert_2^2 \big)\Big) ,
%\end{align}
%where $\epsilon_r$ is the tolerance used to set number of iterations $S_r$ in Proposition \ref{prop:RL-LQG}, then, with probability at least $1 - \epsilon^5$, $F^{(r)} \in \FF$ and $K^{(1,r)}$ is a stabilizing controller for system $(\bar{A}^{(r)}, \bar{B})$ for $1 \leq r \leq R$, and
%\begin{align*}
%& \lVert F^{(R)} - F^* \rVert_2 \leq \epsilon, \lVert K^{(S_R,R)} - K^* \rVert_2 \leq (1 + D_0 ) \epsilon, \\
%& \hspace{0.8cm} J(K^{(S_R,R)},F^{(R)}) - J(K^*,F^*) \leq D_1 \epsilon ,
%\end{align*}
%where $D_0$, $D_1$ are constants, $F^*$ is the equilibrium mean-field state matrix, and $K^*$ is the equilibrium controller for the LQ-MFG. 
%\end{theorem}
%\end{blockremove}
\begin{proof}
	{Let us first split $\lVert F^{(r+1)} - F^* \rVert_2$ using the 
		quantity 
		$\bar{F}^{(r+1)} = \Fs(F^{(r)})$,
		\begin{align} \label{eq:triangle_Fd+1}
		\lVert F^{(r+1)} - F^* \rVert_2 \leq \lVert F^{(r+1)} - \bar{F}^{(r+1)} \rVert_2 + \lVert \bar{F}^{(r+1)} - F^* \rVert_2 .
		\end{align}
		First we bound the term $\lVert \bar{F}^{(r+1)} - F^* \rVert_2 $:
		\begin{align} \label{eq:F_bar_d+1}
		\lVert \bar{F}^{(r+1)} - F^* \rVert_2 = \lVert \Fs(F^{(r)}) - \Fs(F^*) \rVert \leq T_P \lVert F^{(r)} - F^* \rVert_2 .
		\end{align}}
	As for the first term in \eqref{eq:triangle_Fd+1}, we know from the definition of state aggregator \eqref{eq:state_agg} that
	\begin{align*}
	& F^{(r+1)} = A - B (K^{(S_r,r)}_1 + K^{(S_r,r)}_2) , \\ 
	& \bar{F}^{(r+1)} = A - B (K^{(*,r)}_1 + K^{(*,r)}_2) .
	\end{align*}
	{Then,
		\begin{align} \label{eq:F_d+1}
		& \lVert F^{(r+1)} - \bar{F}^{(r+1)} \rVert_2 \nonumber \\
		& \leq \lVert B \rVert_2 \big( \lVert K^{(S_r,r)}_1 - K^{(*,r)}_1 
		\rVert_2 + \lVert K^{(S_r,r)}_2 - K^{(*,r)}_2 \rVert_2 \big) \nonumber\\
		%	& \leq \sqrt{2} \lVert B \rVert_2 \lVert K^{(S_r,r)} - K^{(*,r)} \rVert_2 \nonumber \\
		& \leq \sqrt{2}\lVert B \rVert_2 \lVert K^{(S_r,r)} - K^{(*,r)} \rVert_F \nonumber\\
		%		& \leq \lVert B \rVert_2 \sqrt{ 2 \sigma_{\min}^{-1}(\Sigma_X) \sigma_{\min}^{-1} (C_U) \epsilon_r } \leq \epsilon   2^{-r-2} .
		& \leq \lVert B \rVert_2 \sqrt{ 2 \kappa_3 \epsilon_r } \leq \epsilon   2^{-r-2} .
		\end{align}
		The inequality holds with probability at least $1 - \epsilon^{10}$. The third inequality is due to Proposition \ref{prop:RL-LQG} and the last inequality is due to choice of $\epsilon_r$. Hence using \eqref{eq:F_bar_d+1} and \eqref{eq:F_d+1},
		\begin{align*}
		\lVert F^{(r+1)} - F^* \rVert_2 \leq T_P \lVert F^{(r)} - F^* \rVert_2 + \epsilon 2^{-r-2},
		\end{align*}
		which holds with probability $1 - \epsilon^{10}$. Furthermore with a union bound argument with $R = \Os(\epsilon^{-5})$, %$R = \Os (\log(1 / 
		%\epsilon))$ as 
		%in  
		%\cite{fu2019actor} 
		it holds with probability $1-\epsilon^{5}$,
		\begin{align*}
		\lVert F^{(R)} - F^* \rVert_2 \leq T_P^R \lVert F^{(1)} - F^* \rVert_2 + \epsilon/2 .
		\end{align*}
		As $T_P < 1$ (Assumption \ref{asm:boundforcontract}) and $R$ is defined as in the statement of the theorem, we arrive at \kznote{this sentence is too long, does not read clear to me.}\aznote{edited}
		\begin{align} \label{eq:final_bound_F}
		\lVert F^{(R)} - F^* \rVert_2 \leq \epsilon ,
		\end{align}
		with probability at least $1 - \epsilon^{5}$.} {Now we prove that 
		$F^{(r)} \in \FF$ for $1 \leq r \leq R$ using recursion. Let 
		$F^{(r)} \in \FF$ for $0 \leq r < R$; then, we can prove that $F^{(r+1)} 
		\in \FF$ with probability at 
		least $1 - \epsilon^{10}$,
		\begin{align*}
		& \lVert F^{(r+1)} \rVert_2 \leq \lVert F^{(r+1)} - \bar{F}^{(r+1)} \rVert_2 + \lVert \bar{F}^{(r+1)} \rVert_2 \\
		& \leq \lVert B \rVert_2 \sqrt{ 2 \kappa_3 \epsilon_r } + T_P \leq (1+T_P)/2
		\end{align*}
		with probability at least $1 - \epsilon^{10}$. The second inequality is 
		due to \eqref{eq:F_d+1} and Lemma \ref{lem:F_contract}. Hence 
		$F^{(r)} \in 
		\FF$ for $1 \leq r \leq R$ with probability at least $1 - 
		\epsilon^{5}$ using a union bound argument.} 
	
	Now we 	prove the second inequality in the statement of the Theorem. Using the 	triangle inequality,
	\begin{align*}
	\lVert K^{(S_R,R)} - K^* \rVert_2 \leq & \lVert K^{(S_R,R)} - K^{(*,R)} 
	\rVert_2 
	+ \\
	& \lVert K^{(*,R)} - K^* \rVert_2 .
	\end{align*}
	\kzstrike{be careful with punctuations... a sentence should end with a period (u previously had a comma.).}
	From Proposition \ref{prop:RL-LQG} we know that,
	\begin{align*}
	\lVert K^{(S_R,R)} - K^{(*,R)} \rVert_2 \leq \sqrt{ \kappa_3 \epsilon_R} \leq \epsilon ,
	\end{align*}
	with probability at least $1 - \epsilon^{10}$. Using \eqref{eq:u_t}, \eqref{eq:costate} and linearity of the mean-field trajectory $\bar{Z}^{(R)}$, %$K^{(*,R)}$ 
	%can be defined as,
	\begin{align*}
	K^{(*,R)} = \Bigg[ G_P P A  \hspace{0.3cm} -G_P \sum_{s=0}^{\infty} H_P^s C_Z \big(F^{(R)}\big)^{s+1} \Bigg] .
	\end{align*}
	Similarly, $K^*$ can be defined as,
	\begin{align*}
	K^* = \Bigg[ G_P P A  \hspace{0.3cm} -G_P \sum_{s=0}^{\infty} H_P^s C_Z (F^*)^{s+1} \Bigg] .
	\end{align*}
	Using these definitions,
	\begin{align*}
	& \lVert K^{(*,R)} - K^* \rVert_2 \leq \\
	& \lVert G_P \rVert_2 \sum_{s=0}^{\infty} \lVert H_P \rVert_2^s \lVert C_Z \rVert_2 \lVert \big(F^{(R)}\big)^{s+1} - (F^*)^{s+1} \rVert_2.
	\end{align*}
	\kzstrike{same here. punctuations. I have changed it. check all.}
	Using techniques similar to \azedit{ \eqref{eq:prop_1_work}, in} the proof of Proposition \ref{lem:exist_unique_linear}, we obtain, \kzstrike{which technique? which line/equation are u referring to?}
	\begin{align*}
	\lVert K^{(*,R)} - K^* \rVert_2 & \leq D_0 \lVert F^{(R)} - F^* \rVert_2 \leq D_0 \epsilon,
	\end{align*}
	with probability at least $1 - \epsilon^{5}$, where $D_0 := \frac{\lVert G_P \rVert_2 \lVert C_Z	\rVert_2 }{(1 - \lVert H_P \rVert_2)^2}$. The last inequality is due to \eqref{eq:final_bound_F}, and thus we obtain,
	\begin{align} \label{eq:final_bound_K}
	\lVert K^{(S_R,R)} - K^* \rVert_2 \leq (1 + D_0 ) \epsilon ,
	\end{align}
	with probability at least $1 - \epsilon^{5}$. {Now we prove that $K^{(1,r+1)}$ is a stabilizing controller for system $(\bar{A}^{(r+1)}, \bar{B})$ given $K^{(1,r)}$ is a stabilizing controller for system $(\bar{A}^{(r)}, \bar{B})$ for $0 \leq r < R$}. {We know from \cite{yang2019global} that for any stabilizing $K$,
	\begin{align} \label{eq:def_J}
	J(K,F) = \tr \big( \big(C_X + K^T C_U K \big) \Sigma_K \big) + \sigma^2 \tr(C_U) ,
	\end{align}
	where $\Sigma_K$ is the covariance matrix for the stationary distribution induced by $K$ and is the unique positive definite solution to the Lyapunov equation,}
	\begin{align*}
	\Sigma_K = \Sigma_X + \big(\bar{A} - \bar{B} K \big) \Sigma_K \big(\bar{A} - \bar{B} K \big)^T.
	\end{align*}
	\kzstrike{format is not correct here...}\aznote{edited}. Hence $\Sigma_K$ satisfies,
	\begin{align} \label{eq:def_sigma_k}
	\Sigma_K & = \sum_{t=0}^{\infty} \big(\bar{A} - \bar{B} K \big)^t \Sigma_X \big(\big(\bar{A} - \bar{B} K \big)^t\big)^T \nonumber \\
	& = \sum_{t=0}^{\infty} \big(A - B K_1 \big)^t \Sigma^{11}_X \big(\big(A - B K_1 \big)^t\big)^T , 
	\end{align}
	where $\Sigma^{11}_X = \Sigma_{w} + \sigma^2 B B^T$. From Proposition \ref{prop:RL-LQG} we know that since $K^{(1,r)}$ is stabilizing controller for system $(\bar{A}^{(r)},\bar{B})$, $K^{(S_r,r)}$ is also stabilizing, and hence $J(K^{(S_r,r)}, F^{(r)})$ is finite. Also from Algorithm \ref{alg:actorcritic} we know that $K^{(1,r+1)} = K^{(S_r,r)}$. Using \eqref{eq:def_J} and \eqref{eq:def_sigma_k} we can 	deduce that $J(K^{(1,r+1)}, F^{(r+1)}) = J(K^{(1,r+1)}, F^{(r)})$ as long as 	$F^{(r+1)}$ is stable. This is true with probability at least $1 - \epsilon^{10}$. Finally $J(K^{(1,r+1)}, F^{(r)}) = J(K^{(S_r,r)}, F^{(r)}) < \infty$, and hence $K^{(1,r+1)}$ is a stabilizing controller for system $(\bar{A}	^{(r+1)}, \bar{B})$ for $0 \leq r < R$ with probability at least $1 - \epsilon^{5}$ using a union bound argument.
	
	Now we prove the third inequality from the theorem. For the rest of the proof we will introduce $K^{(R)} := K^{(S_R,R)}$ for conciseness. We begin by obtaining an expression for the cost of a stabilizing controller $K$. Since $K^{(R)}$ and $K^*$ are stabilizing controllers, without any loss of generality, we assume that there exists a $\rho_1$ and $p$ s.t. $\lVert \bar{A} - \bar{B} K^{(R)} \rVert_p \leq \rho_1$ and $\lVert \bar{A} - \bar{B} K^* \rVert_p \leq \rho_1 < 1$. \azedit{Due to the equivalence of $p$ and Frobenius norms, there exist scalars }
	%	From equation \eqref{eq:recur_def_sigma_X} $\Sigma_K$ satisfies,
	%	\begin{align} 
	%	\Sigma_K & = \sum_{t=0}^{\infty} \big(\bar{A} - \bar{B} K \big)^t \Sigma_X 
	%	\big(\big(\bar{A} - \bar{B} K \big)^t\big)^T \nonumber \\
	%	& = \sum_{t=0}^{\infty} \big(A - B K_1 \big)^t \Sigma^{11}_X 
	%	\big(\big(A - B K_1 \big)^t\big)^T ,%\\
	%	%& = \sum_{t=0}^{\infty} L_{K_1}^t \Sigma^{11}_X 
	%	%\big(L_{K_1}^t\big)^T
	%	\end{align}
	%	where $\Sigma^{11}_X = \Sigma_{w} + \sigma^2 B B^T$. 
	Using \eqref{eq:def_J} and \eqref{eq:def_sigma_k}, we can write $J(K^{(R)},F^{(R)})$ and $	J(K^*,F^*)$.
	\begin{align*}
	& J(K^{(R)},F^{(R)}) = \sigma^2 \tr(C_U) + \\
	& \tr \Big( \big( C_X + K^{(R)} C_U \big( K^{(R)} \big)^T \big)\sum_{t=0}^{\infty} L_{R}^t \Sigma^{11}_X \big( L_{R}^t \big)^T \Big) ,\\
	& J(K^{*},F^{*}) = \sigma^2 \tr(C_U) + \\
	& \tr \Big( \big( C_X + K^{*} C_U \big( K^{*} \big)^T \big) \sum_{t=0}^{\infty} L_{*}^t \Sigma^{11}_X \big( L_{*}^t \big)^T \Big) ,
	\end{align*}
	where we have introduced $L_{R}:= A - B K^{(R)}_1$ and $L_{*} := A - B K^{*}_1$. Taking the difference of both terms,
	\begin{align} \label{eq:fin_sample_cost}
	& J(K^{(R)},F^{(R)}) - J(K^{*},F^{*})  \nonumber \\
	& = \tr \Big( \big( C_X + K^{(R)} C_U \big( K^{(R)} \big)^T 	\big)\sum_{t=0}^{\infty} \big(L_{R}^t \Sigma^{11}_X \big( L_{R}^t \big)^T \Big) 	\nonumber\\
	& \hspace{0.4cm} - \tr \Big( \big( C_X + K^{*} C_U \big( K^{*} \big)^T \big) \sum_{t=0}^{\infty} L_{*}^t \Sigma^{11}_X \big( L_{*}^t \big)^T \Big) , \nonumber \\
	& = \tr \Big( \big( C_X + K^{*} C_U \big( K^{*} \big)^T \big) \nonumber \\
	& \sum_{t=0}^{\infty} \big(L_{R}^t \Sigma^{11}_X \big( L_{R}^t \big)^T - L_{*}^t \Sigma^{11}_X \big( L_{*}^t \big)^T \big) \Big) + \nonumber \\
	& \tr\Big( \big( K^{*} C_U \big( K^{*} \big)^T - K^{(R)} C_U \big( K^{(R)} \big)^T \big) \sum_{t=0}^{\infty} L_{*}^t \Sigma^{11}_X \big( L_{*}^t \big)^T \Big).
	\end{align}
	\kzstrike{comma $\longrightarrow$ period. I did not change.}
	The first term on the RHS of \eqref{eq:fin_sample_cost} can be upper bounded using the fact that $C_X + K^{*} C_U \big( K^{*} \big)^T$ is symmetric: \kznote{in the following equation, where did you define $\|\cdot\|_p$? what does it mean? why do we need $p$-norm here??}
	\begin{align}
	& \big\lVert \big( C_X + K^{*} C_U \big( K^{*} \big)^T \big) \big\rVert_F \nonumber \\
	& \tr \Big(\sum_{t=0}^{\infty} \big(L_{R}^t \Sigma^{11}_X \big( L_{R}^t \big)^T - L_{*}^t \Sigma^{11}_X \big( L_{*}^t \big)^T \big) \Big) \nonumber \\
	& \hspace{2cm} \leq 2m c^F_p \big\lVert \big( C_X + K^{*} C_U \big( K^{*} \big)^T \big) \big\rVert_F \nonumber \\
	& \hspace{2cm} \sum_{t=0}^{\infty} \Big\lVert L_{R}^t \Sigma^{11}_X \big( L_{R}^t \big)^T - L_{*}^t \Sigma^{11}_X \big( L_{*}^t \big)^T \Big\rVert_p .
	\end{align}
	This inequality is due to the fact that for any square matrix $A$ with 	dimension $2m \times 2m$, $\tr(A) \leq \sum_{i,j} \lvert A_{i,j} \rvert \leq 2m \sqrt{\sum_{i,j} (A_{i,j})^2 } = 2m \lVert A \rVert_F \leq 2m c^F_p \lVert A \rVert_p $, where the scalar $c^F_p$ \kznote{what is this scalar?} enters due to the equivalence between $p$ and $F$ norms. Now we bound the term,
	\begin{align} \label{eq:cost_term_1}
	& \sum_{t=0}^{\infty} \Big\lVert L_{R}^t \Sigma^{11}_X \big( L_{R}^t \big)^T - L_{*}^t \Sigma^{11}_X \big( L_{*}^t \big)^T \Big\rVert_p \nonumber \\
	& = \sum_{t=0}^{\infty} \Big\lVert L_{R}^t \Sigma^{11}_X \big( L_{R}^t - L_{*}^t \big)^T + \big( L_{R}^t -  L_{*}^t \big) \Sigma^{11}_X \big( L_{*}^t \big)^T \Big\rVert_p \nonumber \\
	& \leq \big\lVert \Sigma^{11}_X \big\rVert_p \sum_{t=0}^{\infty} \big( 		\big\lVert L_{R} \big\rVert_p^t + \big\lVert L_{*} \big\rVert_p^t \big)		\big\lVert L_{R}^t - L_{*}^t \big\rVert_p \nonumber \\
	& \leq \big\lVert \Sigma^{11}_X \big\rVert_p \sum_{t=0}^{\infty} 2 \rho_1^t
	\big\lVert L_{R}^t - L_{*}^t \big\rVert_p \nonumber \\
	& \leq \big\lVert \Sigma^{11}_X \big\rVert_p \sum_{t=0}^{\infty} 2 \rho_1^t \bigg\lVert \sum_{\tau = 0}^{t-1} L_{R}^{t-\tau-1} \big(L_{R} - L_{*} \big) L_{*}^{\tau} \bigg\rVert_p \nonumber \\
	& \leq \big\lVert \Sigma^{11}_X \big\rVert_p 
	\sum_{t=0}^{\infty} 
	2 t \rho_1^{t} \big\lVert L_{R} - L_{*} \big\rVert_p \nonumber \\
	& \leq 2 \frac{\big\lVert \Sigma^{11}_X \big\rVert_p \big\lVert B \big\rVert_p \rho_1}{ (1 - \rho_1)^2}  \big\lVert K^{(R)} - K^* \big\rVert_p \nonumber \\
	& \leq 2 c^p_F \frac{\big\lVert \Sigma^{11}_X \big\rVert_p \big\lVert B \big\rVert_p \rho_1}{ (1 - \rho_1)^2}  \big\lVert K^{(R)} - K^* \big\rVert_F .
	%& = \sum_{t=0}^{\infty} \Big\lVert \big( L_{R}^t - L_{*}^t + L_{*}^t \big) 
	%\Sigma^{11}_X \big( L_{R}^t - L_{*}^t + L_{*}^t \big)^T \\
	%& \hspace{0.2cm} - L_{*}^t \Sigma^{11}_X 
	%\big( L_{*}^t \big)^T \Big\rVert_F \\
	%& \leq \sum_{t=0}^{\infty} \Big\lVert \big( L_{R}^t - L_{*}^t \big) 
	%\Sigma^{11}_X \big( L_{R}^t - L_{*}^t \big)^T + \big( L_{R}^t - L_{*}^t 
	%\big) 
	%\Sigma^{11}_X \big( L_{*}^t \big)^T \\
	%& + L_{*}^t 
	%\Sigma^{11}_X \big(L_{R}^t -  L_{*}^t \big)^T \Big\rVert_F \\
	%& \leq \big\lVert \Sigma^{11}_X \big\rVert_F \sum_{t=0}^{\infty} 
	%\big\lVert 
	%L_{R}^t - L_{*}^t \big\rVert_F^2 + 2 \big\lVert L_{R}^t - L_{*}^t 
	%\big\rVert_F 
	%\big\lVert L_{*} \big\rVert_F^t
	\end{align}
	%Hence the first term in the RHS of equation \eqref{eq:fin_sample_cost} can 
	%be 
	%upper bounded by,
	%\begin{align*}
	%D_1 \big\lVert K^{(R)} - K^* \big\rVert_F ,
	%\end{align*}
	%where,
	%\begin{align*}
	%D_1 = 4m c^F_p c^p_F \frac{\big\lVert C_X + K^{*} C_U \big( K^{*} \big)^T 
	%\big\rVert_F \big\lVert \Sigma^{11}_X \big\rVert_p \big\lVert B 
	%\big\rVert_p}
	%{\rho_1 (1 - \rho_1^2)} .
	%\end{align*}
	The first inequality is obtained using the triangle inequality and the definition of $\rho_1$. The second inequality is obtained by following a procedure similar to that in the proof of Proposition \ref{lem:exist_unique_linear}. Now we upper bound the second term in \eqref{eq:fin_sample_cost}:
	\begin{align} \label{eq:cost_term_2}
	& \hspace{-0.3cm} \tr\Big( \big( K^{*} C_U \big( K^{*} \big)^T - K^{(R)} C_U 
	\big( K^{(R)} \big)^T \big) \sum_{t=0}^{\infty} L_{*}^t \Sigma^{11}_X 
	\big( L_{*}^t \big)^T \Big) \nonumber \\
	& \leq \big\lVert K^{*} C_U \big( K^{*} \big)^T - K^{(R)} C_U \big( K^{(R)} 
	\big)^T \big\rVert_F \nonumber \\
	& \hspace{4cm} \tr\Big(\sum_{t=0}^{\infty} L_{*}^t \Sigma^{11}_X 
	\big( L_{*}^t \big)^T \Big) .
	\end{align}
	The inequality is due to the fact that $K^{*} C_U \big( K^{*} \big)^T - 
	K^{(R)} 
	C_U \big( K^{(R)} 
	\big)^T$ is symmetric. The summation can be upper bounded as follows:
	\begin{align} \label{eq:cost_term_3}
	& \tr\Big(\sum_{t=0}^{\infty} L_{*}^t \Sigma^{11}_X \big( 
	L_{*}^t \big)^T \Big) = \sum_{t=0}^{\infty} \lVert L_{*}^t (\Sigma^{11}
	_X)^{\frac{1}{2}} \rVert_F^2 \nonumber \\
	& \leq c^F_p \sum_{t=0}^{\infty} \lVert L_{*}^t (\Sigma^{11}
	_X)^{\frac{1}{2}} \rVert_p^2 \leq \frac{c^F_p \lVert (\Sigma^{11}
		_X)^{\frac{1}{2}} \rVert_p^2}{1 - \rho_1^2} .
	\end{align}
	The first term in \eqref{eq:cost_term_2} can be upper bounded by,
	\begin{align} \label{eq:cost_term_4}
	& \big\lVert K^{(R)} C_U \big( K^{(R)} 
	\big)^T - K^{*} C_U \big( K^{*} \big)^T \big\rVert_F \nonumber \\
	& = \big\lVert \big(K^{(R)} - K^* + K^* \big) C_U \big( K^{(R)} - K^* + K^*
	\big)^T \nonumber\\
	& \hspace{0.4cm} - K^{*} C_U \big( K^{*} \big)^T \big\rVert_F \nonumber\\
	& = \big\lVert \big(K^{(R)} - K^* \big) C_U \big( K^{(R)} - K^*\big)^T + 
	\nonumber\\
	& \hspace{0.4cm}  2 \big(K^{(R)} - K^* \big) C_U \big( K^* \big)^T 
	\big\rVert_F 
	\nonumber\\
	& \leq \big\lVert C_U \big\rVert_F \Big[ \big\lVert K^{(R)} - K^* 
	\big\rVert_F^2 
	+ 2 \lVert K^* \rVert_F \big\lVert K^{(R)} - K^* \big\rVert_F \Big] .
	\end{align}
	Hence, the difference in costs $J(K^{(R)},F^{(R)}) - J
	(K^{*},F^{*})$ 
	using \eqref{eq:fin_sample_cost}-\eqref{eq:cost_term_4} is
	\begin{align} \label{eq:cost_term_5}
	& J(K^{(R)},F^{(R)}) - J(K^{*},F^{*}) \leq \nonumber \\
	& \hspace{1.5cm}  D_2 \big\lVert K^{(R)} - K^* \big\rVert_F + D_3 \big\lVert 
	K^{(R)} - K^* \big\rVert_F^2 ,
	\end{align}
	where $D_2$ and $D_3$ are defined as follows:
	\begin{align} \label{eq:cost_term_6}
	D_2 := & 4m c^F_p \big\lVert \big( C_X + K^{*} C_U \big( K^{*} \big)^T \big) \big\rVert_F c^p_F \frac{\big\lVert \Sigma^{11}_X \big\rVert_p \big\lVert B \big\rVert_p \rho_1}{ (1 - \rho_1)^2} \nonumber \\
	& + 2 \lVert K^* \rVert_F \big\lVert C_U \big\rVert_F \frac{c^F_p \lVert \Sigma^{11}_X)^{\frac{1}{2}} \rVert_p^2}{1 - \rho_1^2} , \nonumber \\
	D_3 := & \big\lVert C_U \big\rVert_F \frac{c^F_p \lVert (\Sigma^{11}_X)^{\frac{1}{2}} \rVert_p^2}{1 - \rho_1^2} .
	\end{align}
	Using \eqref{eq:final_bound_K}, \eqref{eq:fin_sample_cost}-\eqref{eq:cost_term_6}\kznote{spacing issue.} for $\epsilon$ small enough, with probability at 
	least $1 
	- \epsilon^{5}$,
	%\begin{align*}
	%& J(K^{(R)},F^{(R)}) - J(K^{*},F^{*}) \leq \\
	%&  \hspace{2cm} D_2 \big(1 + D_0 \big) \epsilon + D_3 \big(1 + D_0 \big)^2 
	%\epsilon^2 .
	%\end{align*}
	%For $\epsilon \leq 1$,
	\begin{align*}
	& J(K^{(R)},F^{(R)}) - J(K^{*},F^{*}) \leq D_1 \epsilon,\\
	& \text{ where }D_1 := D_2 \big(1 + D_0 \big) + D_3 \big(1 + D_0 \big)^2 .
	\end{align*}\kznote{can we make $\qed$ be the same line with the ending? you can add an inline  sentence here.}
\end{proof}

%\begin{proof}[Proof Sketch]
%First we prove the bound on $\lVert F^{(R)} - F^* \rVert_2$. We begin with upper bounding the quantity $\lVert F^{(r+1)} - F^* \rVert_2$. This quantity is split into $\lVert F^{(r+1)} - \bar{F}^{(r+1)} \rVert_2 + \lVert \bar{F}^{(r+1)} - F^* \rVert_2$ where $\bar{F}^{(r+1)} = \Ts(F^{(r)})$. First we bound the second term, $\lVert \bar{F}^{(r+1)} - F^* \rVert_2 = \lVert \Ts(F^{(r)}) - \Ts(F^*) \rVert \leq T_P \lVert F^{(r)} - F^* \rVert_2$. The inequality is due to the fact that $\Ts$ is contractive with coefficient $T_P$, from proof of Proposition \ref{lem:exist_unique_linear}. Using the definition of state aggregator \eqref{eq:state_agg}, Proposition \ref{prop:RL-LQG} and definition of $\epsilon_r$ in the statement of Theorem \ref{thm:conv_guarantee}, we deduce, $\lVert F^{(r+1)} - \bar{F}^{(r+1)} \rVert_2 \leq \epsilon  2^{-r-2}$ with high probability. Consequently, $\lVert F^{(r+1)} - F^* \rVert_2 \leq T_P \lVert F^{(r)} - F^* \rVert_2 + \epsilon 2^{-r-2}$ with high probability. Using union bound type argument, we arrive at $\lVert F^{(R)} - F^* \rVert_2 \leq \epsilon$ with high probability. To prove $F^{(r)} \in \FF$ for $r \in [R]$, we use a recursive argument. Let $F^{(r)} \in \FF$ for $r \in [R]$; using Proposition \ref{prop:RL-LQG} and Lemma \ref{lem:F_contract}, we obtain $\lVert F^{(r+1)} \rVert_2 \leq (1+T_P)/2$, and hence $F^{(r+1)} \in \FF$ with high probability. Using union bound type argument, we conclude that $F^{(r)} \in \FF$ for $r \in [R]$ with high probability.
%
%Moving onto the second bound, $\lVert K^{(S_R,R)} - K^* \rVert_2$ is split into $\lVert K^{(S_R,R)} - K^{(*,R)} \rVert_2$ and $\lVert K^{(*,R)} - K^* \rVert_2$. Using Proposition \ref{prop:RL-LQG}, $\lVert K^{(S_R,R)} - K^{(*,R)} \rVert_2 \leq \epsilon$ with probability at least $1 - \epsilon^{10}$. Using the definition of $K^{(*,R)}$, $K^*$, and techniques similar to proof of Proposition \ref{lem:exist_unique_linear}, $\lVert K^{(*,R)} - K^* \rVert_2 \leq D_0 \epsilon,$ where $D_0 := \frac{\lVert G_P \rVert_2 \lVert C_Z	\rVert_2 }{(1 - \lVert H_P \rVert_2)^2}$ with high probability. Hence we conclude that $\lVert K^{(S_R,R)} - K^* \rVert_2 \leq (1 + D_0 ) \epsilon$ with probability at least $1 - \epsilon^{5}$. 
%To prove that $K^{(1,r)}$ is a stabilizing controller for $(\bar{A}^{(r)},\bar{B})$ for $1 \leq r \leq R$, we use a recursive argument. Let $K^{(1,r)}$ be the stabilizing controller for $(\bar{A}^{(r)},\bar{B})$; then, with high probability, $K^{(S_r,r)}$ is also a stabilizing controller for $(\bar{A}^{(r)},\bar{B})$ using Proposition \ref{prop:RL-LQG}. From Algorithm \ref{alg:actorcritic} we know that $K^{(1,r+1)} = K^{(S_r,r)}$. Using the definition of $J(K,F)$, it can be shown that $J(K^{(1,r+1)}, F^{(r+1)}) = J(K^{(1,r+1)}, F^{(r)})$, and hence $K^{(1,r+1)}$ is a stabilizing control for $(\bar{A}^{(r+1)},\bar{B})$. As a result, using a union bound type argument, we conclude that $K^{(1,r)}$ is a stabilizing controller for system $(\bar{A}^{(r)}, \bar{B})$ for $1 \leq r \leq R$ with high probability. 
%For the last bound, using definition of $J(K,F)$, the fact that $K^{(R)} = K^{(S_R,R)}$ and $K^*$ are stable, we can deduce,
%$ J(K^{(R)},F^{(R)}) - J(K^{*},F^{*}) \leq D_2 \big\lVert K^{(R)} - K^* \big\rVert_F + D_3 \big\lVert K^{(R)} - K^* \big\rVert_F^2$, where $D_2$ and $D_3$ are constants. Hence, using the bound $\lVert K^{(R)} - K^* \rVert_2 \leq (1 + D_0 ) \epsilon$, we arrive at $J(K^{(R)},F^{(R)}) - J(K^{*},F^{*}) \leq D_1 \epsilon, $ with high probability.
%\end{proof}
\subsection{Approximate $\epsilon$-NE bound}
We now quantify how the approximate MFE obtained from Theorem 
\ref{thm:conv_guarantee} performs in the original finite population game. Let us denote the control law generated by the approximate MFE $(F^{(R)}, K^{(S_R,R)})$ in Algorithm \ref{alg:actorcritic} by $\tilde{\mu}$. The approximate MFE controller is 
\begin{align}
\tilde{\mu}_t^n(Z^n_t) = - K^{(S_R,R)}_1 Z^n_t - K^{(S_R,R)}_2 (F^{(R)})^t \nu_0
\end{align}
and $\tilde{\mu}^{-n} = (\tilde\mu^1, \ldots,\tilde\mu^{n-1},\tilde\mu^{n+1},\ldots,\tilde\mu^{(N)})$.

%\emedit{The performance of mean-field strategies in the finite-agent game is quantified by the () bound derived in}

\begin{theorem} \label{thm:fin_agent_bound}
Let the output cost of Algorithm \ref{alg:actorcritic} for a finite population LQ game for agent $n$ be $J^N_n (\tilde{\mu}^n, \tilde{\mu}^{-n})$, and denote the NE cost of this game by $\inf_{\pi^n \in \Pi} J^N_n(\pi^n,\tilde{\mu}^{-n})$. Then, 
%suppose $N = \Omega(1/\epsilon^2)$, then after $R = \Omega(\log(1/\epsilon))$ iterations of the outer loop of Algorithm \ref{alg:actorcritic}, we have 
%\begin{align*}
%J^N_n (K^{(S_R,R)},F^{(R)}) - J^N_n (K^*, F^*) \leq \epsilon.
%\end{align*}
if $R = \Omega(\log(1/\epsilon))$ and $N = \Omega(1/\epsilon^2)$,
\begin{align*}
J^N_n (\tilde{\mu}^n, \tilde{\mu}^{-n}) - \inf_{\pi^n \in \Pi} J^N_n(\pi^n,\tilde{\mu}^{-n}) \leq \epsilon .
\end{align*}
with probability at least $1-\epsilon^5$. \kznote{two issues: 1. why dont u put it in the beginning? the notation appears in the first sentence of the theorem, but without introduction; 2. as you already have defined $\tilde{\mu}$, why dont you just say $\tilde{\mu}^n=\tilde{\mu}$ for all $n\in[N]$, and $\tilde{\mu}^{-n}$ denotes the joint policy of all agents except agent $i$? check how saldi's paper used this term...}
%where $\tilde\mu := 
%\mu^{(R)}$ is the controller output by Algorithm 
%\ref{alg:actorcritic} and $\Pi$ is the set of all centralized control 
%laws.
%where $n$ is the number of agents and $S$ is the number of iterations of the 
%outer loop of the RL algorithm.
%$\Os(1/\sqrt{n} )$
\end{theorem}
%\issue{the result u show is not ``$\epsilon$-NE''; also, what is the $K^*$ and $F^*$ here? Does $J^N_n (K^*, J^*)$ make sense in the finite-agent game?} 
\begin{proof}
	The quantity $J^N_n (\tilde{\mu}^n, \tilde{\mu}^{-n}) - \inf_{\pi^n \in \Pi} 
	J^N_n(\pi^n, \tilde{\mu}^{-n})$ can be broken up into two terms,
	\begin{align} \label{eq:exp1_thm11}
	& J^N_n (\tilde{\mu}^n, \tilde{\mu}^{-n}) - \inf_{\pi^n \in \Pi} 
	J^N_n(\pi^n, \tilde{\mu}^{-n}) = \nonumber \\
	& \hspace{1cm} J^N_n (\tilde{\mu}^n, \tilde{\mu}^{-n}) - J(K^{(S_R,R)},F^{(R)}) + \nonumber \\
	& \hspace{1cm} J(K^{(S_R,R)},F^{(R)}) - \inf_{\pi^n \in \Pi} J^N_n(\pi^n, \tilde{\mu}^{-n})
	\end{align}
	For simplicity let us denote $\bar{Z}$ as the mean-field trajectory and $\bar{Z}^N_{n}= (\bar{Z}^N_{n,0}, \bar{Z}^N_{n,1}, \ldots)$ where $\bar{Z}^N_{n,t} = \frac{1}{N-1} \sum_{n' \neq n} Z^{n'}_t$ as the empirical mean-field trajectory under the control law $\tilde{\mu}$. Similarly, denote the trajectory of agent $n$ under control law $\pi^n \in \Pi$ by $Z^n_t$. %where, $\pi^n$ minimizes the finite population cost, $J^N_n(\pi^n, \tilde{\mu}^{-n}) \leq J^N_n(\pi, \tilde{\mu}^{-n}), $ for any $ \pi \in \Pi$. 
	Using Lemma 3 in \cite{moon2014discrete}, since it is applicable for any stabilizing controller,
	\begin{align} \label{eq:exp1_thm21}
	& J^N_n (\tilde{\mu}^n, \tilde{\mu}^{-n}) - J(K^{(S_R,R)},F^{(R)}) = \nonumber \\
	& \hspace{1cm} \Os \Bigg( \sqrt{\limsup_{T \rightarrow \infty} \EE_{\tilde{\mu}} \big( \sum_{t=0}^{T-1} \big\lVert \bar{Z}^{N}_{n,t} - \bar{Z}_t \big\rVert_2^2 \big)/T} \Bigg) .
	\end{align}
	Now we obtain an upper bound for the expression on the RHS. Using \eqref{eq:finitesystem} the dynamics of $\bar{Z}^{N}_{n}$ can be written as
	\begin{align*}
	\bar{Z}^{N}_{n,t+1} = (A - B K_1^{(S_R,R)}) \bar{Z}^{N}_{n,t} - B K_2^{(S_R,R)} \bar{Z}_t + W^{N}_{n,t},
	\end{align*}
	where $W^{N}_{n,t} := \sum_{n' \neq n} (W^{n'}_t + B \zeta^{n'})/(N-1)$, 
	is generated i.i.d. with distribution $\Ns(0,\Sigma^N_w)$ where $\Sigma^N_w = \frac{\Sigma_w + \sigma^2 B B^T}{N-1}$ and $\EE [\bar{Z}^{N}_{n,0}] = \nu_0$. If we augment the states $\bar{Z}^{N}
	_{n,t}$ and $\bar{Z}_t$, the state dynamics of this augmented system can be written as
	\begin{align*}
	\left( \begin{array}{c}
	\bar{Z}^{N}_{n,t+1} \\ \bar{Z}_{t+1}\end{array} \right) = \big(\bar{A} - \bar{B} K^{(S_R,R)}\big) \left( \begin{array}{c}\bar{Z}^{N}_{n,t} \\ \bar{Z}_{t} \end{array} \right) + \left( \begin{array}{c}W^{N}_{n,t} \\ 0\end{array} \right) ,
	\end{align*}
	and the expression inside the parenthesis on the RHS of \eqref{eq:exp1_thm21} can be expressed as the cost function, \kzstrike{summation to $T-1$?? plz be careful and check all.}
	\begin{align*} %\label{eq:cost_in_proof}
	%& \limsup_{T \rightarrow \infty} \frac{1}{T} \EE \big( \sum_{t=0}^{T} 
	%\big\lVert \Delta^{N}_{n,t}\big\rVert_2^2 \big) = \nonumber \\
	& \limsup_{T \rightarrow \infty} \frac{1}{T} \EE_{\tilde{\mu}} \bigg( \sum_{t=0}^{T-1} \bigg\lVert \begin{array}{c}\bar{Z}^{N}_{n,t} \\ \bar{Z}_{t}\end{array} \bigg\rVert_D^2 \bigg) \text{ where } D = \left( \begin{array}{cc} I & -I \\ -I & I \end{array} \right) .
	\end{align*}
	Since $K^{(S_R,R)}$ is a stabilizing controller for system $(\bar{A}, \bar{B})$, using Proposition 3.1 from \cite{yang2019global}, we know that the cost in equation above is $\Os(\tr(\Sigma^N_w)) = \Os(1/(N-1))$. Hence,
	\begin{align} \label{eq:bound_finite_vs_infty1}
	\sqrt{\limsup_{T \rightarrow \infty} \EE_{\tilde{\mu}} \big( \sum_{t=0}^{T-1} \big\lVert \bar{Z}^{N}_{n,t} - \bar{Z}_t \big\rVert_2^2 \big)/T} = \Os \bigg( \frac{1}{\sqrt{N-1}} \bigg).
	\end{align}
	
	Next we use the approach of Lemma 4 in \cite{moon2014discrete} to obtain an upper bound on $J(K^{(S_R,R)},F^{(R)}) - J^N_n(\pi^n, \tilde{\mu}^{-n})$. \kznote{start the equation with a sentence??}\azedit{ The cost for agent $n$ under control law $\pi^n \in \Pi$, while the other agents in the $N$-agent game are following the approximate MFE controller $\tilde{\mu}$ is }
	\begin{align} \label{eq:exp2_thm21}
	& J^N_n(\pi^n,\tilde{\mu}^{-n}) \nonumber \\
	& = \limsup_{T \rightarrow \infty} \frac{1}{T} \sum^{T-1}_{t=0} \EE \big[ \lVert Z^n_t - \bar{Z}_t + \bar{Z}_t - \bar{Z}^N_{n,t} \rVert^2_{C_Z} + \lVert U_t \rVert^2_{C_X} \big] \nonumber \\
	& \geq J(\pi^n,\bar{Z}) + \limsup_{T \rightarrow \infty} \frac{2}{T} \sum_{t=0}^{T-1} \EE \big[ (Z^n_t - \bar{Z}_t)^T C_Z (\bar{Z}_t - \bar{Z}^N_{n,t} \big] \nonumber \\
	& \geq J(K^{(S_R,R)},F^{(R)}) - 2 D_1 \lVert F^{(1)} - F^* \rVert_2 T^R_P + \nonumber \\
	& \hspace{1.5cm} \limsup_{T \rightarrow \infty} \frac{2}{T} \sum_{t=0}^{T-1} \EE \big[ (Z^n_t - \bar{Z}_t)^T C_Z (\bar{Z}_t - \bar{Z}^N_{n,t} \big]
	\end{align}
	with probability at least $1-\epsilon^5$. \kznote{what about the second-to-last inequality? how did u obtain it?} The last inequality is obtained by using the definition of $R$ and the upper bound on $J(K^{(S_R,R)},F^{(R)}) - J(K^*,F^*)$ from Theorem \ref{thm:conv_guarantee}. The last term on the RHS of \eqref{eq:exp2_thm21} can be bounded by techniques used in Lemma 4 in \cite{moon2014discrete}:
	\begin{align} \label{eq:exp3_thm21}
	& \bigg\lvert \limsup_{T \rightarrow \infty} \frac{2}{T} \sum_{t=0}^{T-1} \EE \big[ (Z^n_t - \bar{Z}_t)^T C_Z (\bar{Z}_t - \bar{Z}^N_{n,t} \big] \bigg\rvert = \nonumber \\
	& \hspace{1.5cm} \Os \Bigg( \sqrt{\limsup_{T \rightarrow \infty} \EE_{\tilde{\mu}} \big( \sum_{t=0}^{T-1} \big\lVert \bar{Z}^{N}_{n,t} - \bar{Z}_t \big\rVert_2^2 \big)/T} \Bigg).
	\end{align}
	\kzstrike{missing a period.}
	Using \eqref{eq:bound_finite_vs_infty1}--\eqref{eq:exp3_thm21}, 
	\vspace{-0.15cm}\begin{align} \label{eq:exp4thm21}
	J(K^{(S_R,R)},F^{(R)}) - J^N_n(\pi^n,\tilde{\mu}^{-n}) = \Os \big( T^R_P \big) + \Os \Big( \frac{1}{\sqrt{N-1}} \Big), 
	\end{align}
	with probability at least $1-\epsilon^5$. Now using \eqref{eq:exp1_thm11}, \eqref{eq:exp1_thm21}, \eqref{eq:bound_finite_vs_infty1} and \eqref{eq:exp4thm21} we arrive at,
	\begin{align*}
	J^N_n (\tilde{\mu}^n, \tilde{\mu}^{-n}) - J^N_n(\pi^n,\tilde{\mu}^{-n})= \Os \big( T^R_P \big) + \Os \Big( \frac{1}{\sqrt{N-1}} \Big),
	\end{align*}
	with probability at least $1-\epsilon^5$. Hence if $R = \Omega(\log(1/\epsilon))$ and $N = \Omega(1/\epsilon^2)$, then, with probability at least $1-\epsilon^5$.
	\begin{align*}
	J^N_n (\tilde{\mu}^n, \tilde{\mu}^{-n}) - J^N_n(\pi^n,\tilde{\mu}^{-n}) \leq \epsilon .
	\end{align*}
	for any $\pi^n \in \Pi$ and so the proof is obtained.
	\kznote{adding ``for any $\pi^n \in \Pi$''?}
%	\vspace{-1.1cm}
	%The quantity can be broken up into the following three quantities,
	%\begin{align} \label{eq:final_cost_split}
	%& J^N_n (K^{(S_R,R)},F^{(R)}) - J^N_n (K^*, F^*) \leq \nonumber 
	%\\
	%& \hspace{1.5cm} \big\lvert J^N_n (K^{(S_R,R)},F^{(R)}) - J 
	%(K^{(S_R,R)},F^{(R)}) \big\rvert + \nonumber\\
	%& \hspace{1.5cm} \big\lvert J (K^{(S_R,R)},F^{(R)}) - J (K^*, 
	%F^*) 
	%\big\rvert + \nonumber\\
	%& \hspace{1.5cm} \big\lvert J (K^*, F^*) - J^N_n (K^*, F^*) 
	%\big\rvert .
	%\end{align}
	%The first and 
	%the 
	%third terms are bounded by using Lemma 4 in \cite{moon2014discrete} 
	%since that 
	%lemma deals with any stabilizing controller. This bound is in terms of 
	%the difference between the empirical mean-field trajectory $\bar{Z}^{(N)}_{n}$
	%(aggregate 
	%behavior in finite agent case) and 
	%the mean-field trajectory $\bar{Z}$. By writing down the 
	%dynamics 
	%of $\bar{Z}^{(N)}_{n}$ and $\bar{Z}$ and augmenting them we 
	%achieve an LQG system with a stabilizing control. Using cost of a 
	%stabilizing controller from \cite{yang2019global} the first and third terms in 
	%equation \eqref{eq:final_cost_split} are bounded. The second term in 
	%\eqref{eq:final_cost_split} is bounded by using Theorem \ref{thm:conv_guarantee}
	
\end{proof}

%\begin{proof}[Proof Sketch]
%The quantity $J^N_n (\tilde{\mu}^n, \tilde{\mu}^{-n}) - \inf_{\pi^n \in \Pi} 
%J^N_n(\pi^n, \tilde{\mu}^{-n})$ can be broken up into two terms,
%{\small \begin{align} \label{eq:exp1_thm11}
%& J^N_n (\tilde{\mu}^n, \tilde{\mu}^{-n}) - \inf_{\pi^n \in \Pi} 
%J^N_n(\pi^n, \tilde{\mu}^{-n}) = \nonumber \\
%& \hspace{1cm} J^N_n (\tilde{\mu}^n, \tilde{\mu}^{-n}) - J(K^{(S_R,R)},F^{(R)}) + \nonumber \\
%& \hspace{1cm} J(K^{(S_R,R)},F^{(R)}) - \inf_{\pi^n \in \Pi} J^N_n(\pi^n, \tilde{\mu}^{-n}).
%\end{align}}
%
%For simplicity let us denote $\bar{Z}$ as the mean-field trajectory and $\bar{Z}^N_{n}= (\bar{Z}^N_{n,0}, \bar{Z}^N_{n,1}, \ldots)$ where $\bar{Z}^N_{n,t} = \frac{1}{N-1} \sum_{n' \neq n} Z^{n'}_t$ as the empirical mean-field trajectory under the control law $\tilde{\mu}$. Similarly, denote the trajectory of agent $n$ under control law $\pi^n \in \Pi$ by $Z^n_t$. %where, $\pi^n$ minimizes the finite population cost, $J^N_n(\pi^n, \tilde{\mu}^{-n}) \leq J^N_n(\pi, \tilde{\mu}^{-n}), $ for any $ \pi \in \Pi$. 
%Using Lemma 3 in \cite{moon2014discrete}, since it is applicable for any stabilizing controller,
%{\small \begin{align} \label{eq:exp1_thm21}
%& J^N_n (\tilde{\mu}^n, \tilde{\mu}^{-n}) - J(K^{(S_R,R)},F^{(R)}) = \nonumber \\
%& \hspace{1cm} \Os \Bigg( \sqrt{\limsup_{T \rightarrow \infty} \EE_{\tilde{\mu}} \big( \sum_{t=0}^{T-1} \big\lVert \bar{Z}^{N}_{n,t} - \bar{Z}_t \big\rVert_2^2 \big)/T} \Bigg) .
%\end{align}}
%By defining a vector $Z^N_{n,t} = [(\bar{Z}^{N}_{n,t})^T, \bar{Z}_{t}^T]^T$ the expression inside square root on the RHS of \eqref{eq:exp1_thm21} can be expressed as $\limsup_{T \rightarrow \infty} \EE_{\tilde{\mu}} [ \sum_{t=0}^{T-1} \lVert Z^N_{n,t} \rVert_D^2/T ]$. By expressing the dynamics of $Z^N_{n,t}$, this expression can be shown to be the cost of an LQR system which is $\Os(1/(N-1))$.
%
%Moving to the second expression in the RHS of \eqref{eq:exp1_thm11}, using the definition of $J^N_n(\pi^n,\tilde{\mu}^{-n})$,
%\begin{align} \label{eq:exp2_thm21}
%& J^N_n(\pi^n,\tilde{\mu}^{-n}) \geq J(K^{(S_R,R)},F^{(R)}) - 2 D_1 \lVert F^{(1)} - F^* \rVert_2 T^R_P  \nonumber \\
%& \hspace{0.5cm} + \limsup_{T \rightarrow \infty} \frac{2}{T} \sum_{t=0}^{T-1} \EE \big[ (Z^n_t - \bar{Z}_t)^T C_Z (\bar{Z}_t - \bar{Z}^N_{n,t} \big]
%\end{align}
%with high probability. By techniques used in Lemma 4 in \cite{moon2014discrete}, the last term on the RHS of \eqref{eq:exp2_thm21} can be shown to be $\Os (\sqrt{\limsup_{T \rightarrow \infty} \EE_{\tilde{\mu}} ( \sum_{t=0}^{T-1} \lVert \bar{Z}^{N}_{n,t} - \bar{Z}_t \rVert_2^2 )/T})$, and hence is $\Os(1/\sqrt{N-1})$. Finally, if $R = \Omega(\log(1/\epsilon))$ and $N = \Omega(1/\epsilon^2)$, then by using the logic defined above, with high probability $J^N_n (\tilde{\mu}^n, \tilde{\mu}^{-n}) - J^N_n(\pi^n,\tilde{\mu}^{-n}) \leq \epsilon$.
%%{\color{gray}Now we obtain an upper bound for the expression on the RHS. Using \eqref{eq:finitesystem} the dynamics of $\bar{Z}^{N}_{n}$ can be written as
%%\begin{align*}
%%\bar{Z}^{N}_{n,t+1} = (A - B K_1^{(S_R,R)}) \bar{Z}^{N}_{n,t} - B K_2^{(S_R,R)} \bar{Z}_t + W^{N}_{n,t},
%%\end{align*}
%%where $W^{N}_{n,t} := \sum_{n' \neq n} (W^{n'}_t + B \zeta^{n'})/(N-1)$, 
%%is generated i.i.d. with distribution $\Ns(0,\Sigma^N_w)$ where $\Sigma^N_w = \frac{\Sigma_w + \sigma^2 B B^T}{N-1}$ and $\EE [\bar{Z}^{N}_{n,0}] = \nu_0$. If we augment the states $\bar{Z}^{N}
%%_{n,t}$ and $\bar{Z}_t$, the state dynamics of this augmented system can be written as
%%\begin{align*}
%%\left( \begin{array}{c}
%%\bar{Z}^{N}_{n,t+1} \\ \bar{Z}_{t+1}\end{array} \right) = \big(\bar{A} - \bar{B} K^{(S_R,R)}\big) \left( \begin{array}{c}\bar{Z}^{N}_{n,t} \\ \bar{Z}_{t} \end{array} \right) + \left( \begin{array}{c}W^{N}_{n,t} \\ 0\end{array} \right) ,
%%\end{align*}
%%and the expression inside the parenthesis on the RHS of \eqref{eq:exp1_thm21} can be expressed as the cost function,
%%\begin{align*} %\label{eq:cost_in_proof}
%%%& \limsup_{T \rightarrow \infty} \frac{1}{T} \EE \big( \sum_{t=0}^{T} 
%%%\big\lVert \Delta^{N}_{n,t}\big\rVert_2^2 \big) = \nonumber \\
%%& \limsup_{T \rightarrow \infty} \frac{1}{T} \EE_{\tilde{\mu}} \bigg( \sum_{t=0}^{T} \bigg\lVert \begin{array}{c}\bar{Z}^{N}_{n,t} \\ \bar{Z}_{t}\end{array} \bigg\rVert_D^2 \bigg) \text{ where } D = \left( \begin{array}{cc} I & -I \\ -I & I \end{array} \right) .
%%\end{align*}
%%Since $K^{(S_R,R)}$ is a stabilizing controller for system $(\bar{A}, \bar{B})$, using Proposition 3.1 from \cite{yang2019global}, we know that the cost in equation above is $\Os(\tr(\Sigma^N_w)) = \Os(1/(N-1))$. Hence,
%%\begin{align} \label{eq:bound_finite_vs_infty1}
%%\sqrt{\limsup_{T \rightarrow \infty} \EE_{\tilde{\mu}} \big( \sum_{t=0}^{T} \big\lVert \bar{Z}^{N}_{n,t} - \bar{Z}_t \big\rVert_2^2 \big)/T} = \Os \bigg( \frac{1}{\sqrt{N-1}} \bigg).
%%\end{align}
%%
%%Next we use the approach of Lemma 4 in \cite{moon2014discrete} to obtain an upper bound on $J(K^{(S_R,R)},F^{(R)}) - J^N_n(\pi^n, \tilde{\mu}^{-n})$.
%%\begin{align} \label{eq:exp2_thm21}
%%& J^N_n(\pi^n,\tilde{\mu}^{-n}) \nonumber \\
%%& = \lim_{T \rightarrow \infty} \frac{1}{T} \sum^{T}_{t=0} \EE \big[ \lVert Z^n_t - \bar{Z}_t + \bar{Z}_t - \bar{Z}^N_{n,t} \rVert^2_{C_Z} + \lVert U_t \rVert^2_{C_X} \big] \nonumber \\
%%& \geq J(\pi^n,\bar{Z}) + \lim_{T \rightarrow \infty} \frac{2}{T} \sum_{t=0}^{T} \EE \big[ (Z^n_t - \bar{Z}_t)^T C_Z (\bar{Z}_t - \bar{Z}^N_{n,t} \big] \nonumber \\
%%& \geq J(K^{(S_R,R)},F^{(R)}) - 2 D_1 \lVert F^{(1)} - F^* \rVert_2 T^R_P + \nonumber \\
%%& \hspace{1.5cm} \lim_{T \rightarrow \infty} \frac{2}{T} \sum_{t=0}^{T} \EE \big[ (Z^n_t - \bar{Z}_t)^T C_Z (\bar{Z}_t - \bar{Z}^N_{n,t} \big]
%%\end{align}
%%with probability at least $1-\epsilon^5$. The last inequality is obtained by using the definition of $R$ and the upper bound on $J(K^{(S_R,R)},F^{(R)}) - J(K^*,F^*)$ from Theorem \ref{thm:conv_guarantee}. The last term on the RHS of \eqref{eq:exp2_thm21} can be bounded by techniques used in Lemma 4 in \cite{moon2014discrete}:
%%\begin{align} \label{eq:exp3_thm21}
%%& \bigg\lvert \lim_{T \rightarrow \infty} \frac{2}{T} \sum_{t=0}^{T} \EE \big[ (Z^n_t - \bar{Z}_t)^T C_Z (\bar{Z}_t - \bar{Z}^N_{n,t} \big] \bigg\rvert = \nonumber \\
%%& \hspace{1.5cm} \Os \Bigg( \sqrt{\limsup_{T \rightarrow \infty} \EE_{\tilde{\mu}} \big( \sum_{t=0}^{T} \big\lVert \bar{Z}^{N}_{n,t} - \bar{Z}_t \big\rVert_2^2 \big)/T} \Bigg)
%%\end{align}
%%Using \eqref{eq:bound_finite_vs_infty1}--\eqref{eq:exp3_thm21}, 
%%\vspace{-0.15cm}\begin{align} \label{eq:exp4thm21}
%%J(K^{(S_R,R)},F^{(R)}) - J^N_n(\pi^n,\tilde{\mu}^{-n}) = \Os \big( T^R_P \big) + \Os \Big( \frac{1}{\sqrt{N-1}} \Big), 
%%\end{align}
%%with probability at least $1-\epsilon^5$. Now using \eqref{eq:exp1_thm11}, \eqref{eq:exp1_thm21}, \eqref{eq:bound_finite_vs_infty1} and \eqref{eq:exp4thm21} we arrive at,
%%\begin{align*}
%%J^N_n (\tilde{\mu}^n, \tilde{\mu}^{-n}) - J^N_n(\pi^n,\tilde{\mu}^{-n})= \Os \big( T^R_P \big) + \Os \Big( \frac{1}{\sqrt{N-1}} \Big),
%%\end{align*}
%%with probability at least $1-\epsilon^5$. Hence if $R = \Omega(\log(1/\epsilon))$ and $N = \Omega(1/\epsilon^2)$, then, with probability at least $1-\epsilon^5$.
%%\begin{align*}
%%J^N_n (\tilde{\mu}^n, \tilde{\mu}^{-n}) - J^N_n(\pi^n,\tilde{\mu}^{-n}) \leq \epsilon .
%%\end{align*}
%%
%%
%%%\vspace{-1.1cm}
%%%The quantity can be broken up into the following three quantities,
%%%\begin{align} \label{eq:final_cost_split}
%%%& J^N_n (K^{(S_R,R)},F^{(R)}) - J^N_n (K^*, F^*) \leq \nonumber 
%%%\\
%%%& \hspace{1.5cm} \big\lvert J^N_n (K^{(S_R,R)},F^{(R)}) - J 
%%%(K^{(S_R,R)},F^{(R)}) \big\rvert + \nonumber\\
%%%& \hspace{1.5cm} \big\lvert J (K^{(S_R,R)},F^{(R)}) - J (K^*, 
%%%F^*) 
%%%\big\rvert + \nonumber\\
%%%& \hspace{1.5cm} \big\lvert J (K^*, F^*) - J^N_n (K^*, F^*) 
%%%\big\rvert .
%%%\end{align}
%%%The first and 
%%%the 
%%%third terms are bounded by using Lemma 4 in \cite{moon2014discrete} 
%%%since that 
%%%lemma deals with any stabilizing controller. This bound is in terms of 
%%%the difference between the empirical mean-field trajectory $\bar{Z}^{(N)}_{n}$
%%%(aggregate 
%%%behavior in finite agent case) and 
%%%the mean-field trajectory $\bar{Z}$. By writing down the 
%%%dynamics 
%%%of $\bar{Z}^{(N)}_{n}$ and $\bar{Z}$ and augmenting them we 
%%%achieve an LQG system with a stabilizing control. Using cost of a 
%%%stabilizing controller from \cite{yang2019global} the first and third terms in 
%%%equation \eqref{eq:final_cost_split} are bounded. The second term in 
%%%\eqref{eq:final_cost_split} is bounded by using Theorem \ref{thm:conv_guarantee}
%%}
%\end{proof}

%\begin{theorem}
%The difference between finite agent and infinite agent cost is,
%\begin{align*}
%J(K^*) - J^n_i(K^*) \leq \epsilon
%\end{align*}
%where $n$ is the number of agents and $S$ is the number of iterations of the 
%outer loop of the RL algorithm.
%
%$\Os(1/\sqrt{n} )$
%
%\end{theorem}

%\kzstrike{General comments on the proofs: I think since right now we will have the arxiv version, I suggestion to include ``more details'', and give ``complete proofs'' in the arxiv version. For example, some of the arguments in the current ``proofs'' are a bit handwaving. We need to give more details in the arxiv version.} \azstrike{Ive restated it as proof outline, will include complete proof in ArXiv version}\kzstrike{great. shall we be consistent in using this? sometimes you've used ``Proof sketch'', sometimes ``Proof outline'', sometimes ``Proof''. I think we can all use ``Proof sketch''.}\azstrike{Corrected}




==> Section7.tex <==

We have developed a policy iteration algorithm for approximating equilibria in infinite-horizon LQ-MFGs with discounted cost. The main challenge in the algorithm development arises from the fact that the optimal control is computed backward in time. By investigating properties of the mean-field update operator (which we term the $\tau$-latent property), we can represent the mean-field trajectory at any given iteration by a finite set of parameters, resulting in a forward-in-time construction of the optimal control. The algorithm is provably convergent, with numerical results demonstrating the nature of convergence. The optimality of the computed equilibrium is empirically studied; naturally, the optimality of the approximate equilibrium improves as the iteration index increases and the stopping threshold decreases. 
The results derived in this paper provide an algorithmic viewpoint of the nature of mean-field equilibria for LQ-MFGs. We believe that such insights will be useful for developing model-free  algorithms that improve the scalability of existing  multi-agent RL algorithms in finite-agent settings \cite{zhang18cdc,zhang2018fully}. 




%In this paper we study LQ-MFGs in a discrete-time setting with discounted cost. We develop a \emph{computable} PI algorithm to approximate the mean-field equilibria of the LQ-MFG. This is attained by first introducing a mean-field update operator which, under an assumption on the agent parameters, is shown to be contractive. Then using a property of the mean-field update operator, in conjunction with $\tau$-latent LTI mean-fields, we construct a computable PI algorithm to approximate the mean-field equilibrium of the LQ-MFG. Lastly we show the efficacy of this approximate MFE for different levels of approximation and numbers of agents. Future work includes extension to the model-free setting.







































